A Close Look into the Calibration of Pre-trained Language Models

Pre-trained language models (PLMs) may fail in giving reliable estimates of their predictive uncertainty. We take a close look into this problem, aiming to answer two questions: (1) Do PLMs learn to become calibrated in the training process? (2) How effective are existing calibration methods? For the first question, we conduct fine-grained control experiments to study the dynamic change in PLMs' calibration performance in training. We consider six factors as control variables, including dataset difficulty, available training samples, training steps, the number of tunable parameters, model scale, and pretraining. We observe a consistent change in calibration performance across six factors. We find that PLMs don't learn to become calibrated in training, evidenced by the continual increase in confidence, no matter whether the predictions are correct or not. We highlight that our finding somewhat contradicts two established conclusions: (a) Larger PLMs are more calibrated; (b) Pretraining improves model calibration. Next, we study the effectiveness of existing calibration methods in mitigating the overconfidence issue. Besides unlearnable calibration methods (e.g., label smoothing), we adapt and extend two recently proposed learnable methods that directly collect data to train models to have reasonable confidence estimations. Experimental results show that learnable methods significantly reduce PLMs' confidence in wrong predictions. The code is available at \url{https://github.com/lifan-yuan/PLMCalibration}.

==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/abs.tex <==

\begin{abstract}
% \looseness=-1
Pre-trained language models (PLMs) may fail in giving reliable estimates of their predictive uncertainty. 
% However, well-calibrated PLMs are essential for decision-makers in high-risk applications since their confidence scores reflect the true probability of the outcomes. Given the lack of a comprehensive understanding of PLMs calibration, 
We take a close look into this problem, aiming to answer two questions: (1) Do PLMs learn to become calibrated in the training process? (2) How effective are existing calibration methods? For the first question, we conduct fine-grained control experiments to study the dynamic change in PLMs' calibration performance in training. We consider six factors as control variables, including dataset difficulty, available training samples, training steps, the number of tunable parameters, model scale, and pretraining. We observe a consistent change in calibration performance across six factors. We find that PLMs don't learn to become calibrated in training, evidenced by the continual increase in confidence, no matter whether the predictions are correct or not. We highlight that our finding somewhat contradicts two established conclusions: (a) Larger PLMs are more calibrated; (b) Pretraining improves model calibration. Next, we study the effectiveness of existing calibration methods in mitigating the overconfidence issue. Besides unlearnable calibration methods (e.g., label smoothing), we adapt and extend two recently proposed learnable methods that directly collect data to train models to have reasonable confidence estimations. Experimental results show that learnable methods significantly reduce PLMs' confidence in wrong predictions. The code is available at \url{https://github.com/lifan-yuan/PLMCalibration}.
% and our methods exhibit superior performance compared with previous methods. 


% All the code and data can be obtained at \url{https://github.com/lifan-yuan/PLMCalibration}.




% \yang{Besides, we provide extensions to two existing findings based on our analysis results: (a) PLMs can be trained to output their uncertainty by words; (b) PLMs show degraded performance under distribution shifts.}
% We reveal the potential in learnable methods, by 



% We show that more data and larger model scale for the calibration task can overall improve the calibration performance.



\end{abstract}



% We draw a general conclusion that PLMs' calibration performance is highly determined by their fitness on the training distribution.


% Pre-trained language models (PLMs) achieve super human performance on many downstream tasks, but may fail in giving reliable estimates of their predictive uncertainty. 
% However, well-calibrated models are essential for decision makers in high-risk applications since their confidence scores reflect the true probability of the outcomes.
% To gain a deeper understanding of PLMs calibration, we first conduct a comprehensive empirical study, exploring the influence of six dimensions on PLMs calibration, including dataset difficulty, available training sample, training step, the number of tunable parameter, model scale, and pretraining. 
% We provide a fine-grained conclusion that the calibration performance is highly relevant to PLMs' fitness on the training distribution, which is dynamically influenced by the six dimensions identified above. 
% We observe a continual increase in confidence, no matter the predictions are correct or not, when more fitted on the distribution.
% This results in (1) increasing ECE in the latter ``overfitting'' stage, and (2) continually becoming more confident in wrong predictions in the fitting process. 
% This is partially contradictory to two established conclusions: 
% (1) Larger PLMs are more calibrated;
% (2) Pretraining improves PLMs calibration.
% % We find that there exist some contradictions between our conclusions and the previous ones.
% Next, we move towards practical applications, and investigate existing calibration methods in both in-distribution and various out-of-distribution settings. 
% We identify temperature scaling and label smoothing remain strong baselines for PLMs calibration.
% Besides, we reveal the potential in learnable methods, by directly collecting data to train models to have reasonable confidence estimations.  
% We show that more data and larger model scale can improve the calibration performance. 


% We show that model calibration can be formalized as a task. 
% This task aims to extract features from samples and the model's preceding performance to predict whether a model can give correct answers.


% We show that the size of datasets for the calibration task and model scale both impact the calibration performance from different aspects. 


% we first conduct a fine-grained empirical study, exploring the influence of four factors on model calibration, including the available training samples, fitness on training samples, model capacity, and dataset difficulty. 
% Our comprehensive analysis provides findings of PLMs calibration from multiple dimensions.
% While some of them are consistent with and support previous conclusions, we do provide brand-new, fine-grained, and contradictory findings.
% Given the analysis, we next reexamine two established conclusions: 



% identify four important factors that have a significant influence on model calibration and are overlooked in previous works. 


% we first 
% Next, we decompose the whole pipeline and identify four major factors that have significant infles on model calibration without the interventions of calibration methods, including available training signals, fitness on training samples, model capacity, and dataset difficulty.
% We conduct experiments to empirically prove it by taking a close look into calibration from four dimensions correspondingly.
% , including available training samples, training dynamics, the number of tunable parameters, and the datasets. 

% \yang{discuss emergent calibration: model calibration can be formalized into a task, extracting features from text and predict the uncertainty, given previous history performance.}


% The code will be made public.


==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/calibration_method.tex <==


\input{tab/methods_shift_t5}

\section{How Effective are Existing Methods?}
\looseness=-1
% In this section, we aim to answer the question:
% How effective are existing calibration methods?
% We first describe the experimental settings, and then summarize the conclusions.


% Given our fine-grained understanding of PLMs calibration, we move forwards to situate the PLMs calibration problem in practice, and study existing calibration methods in both in-distribution and out-of-distribution settings.

% \subsection{Experimental setting}
\subsection{Calibration Methods}
% \looseness=-1
\label{sec:cal_method}
We choose representative calibration methods from each category summarized in Sec.~\ref{sec:background}.
% 
For unlearnable methods, we consider vanilla fine-tuning (Vanilla), temperature scaling (TS)~\citep{DBLP:conf/icml/GuoPSW17}, label smoothing (LS)~\citep{DBLP:conf/cvpr/SzegedyVISW16}, easy data augmentation (EDA)~\citep{DBLP:conf/emnlp/WeiZ19}, and deep-ensemble (Ensemble)~\citep{DBLP:conf/nips/Lakshminarayanan17}.
For learnable methods, an extra calibration task is introduced, aiming to train a model to predict whether the original predictions are correct or not.
Each sample in the dataset of the calibration task consists of the original input, the model's original prediction, and the label indicating whether the original prediction is correct or not.
% consists of certain features (e.g., text patterns, the last hidden states) and models' preceding performance.
We adopt the validation set to generate the training set for the calibration task.
% 
We describe the specially designed training paradigms of different methods in the following paragraph and leave the detailed construction process of the calibration training dataset in Appendix~\ref{sec:appendix_construction_of_cal}.
% The detailed processing process is described in Appendix.


\looseness=-1
For better clarification, we use the main task to denote the original task.
The predictive model for the calibration task can be a separate extrinsic model that we use ``E-'' for denotation.
Specifically, we adapt the method proposed in \citet{kadavath2022language} that uses MLP as the extrinsic model (E-MLP) and the inputs are the hidden states of the main task model.
Based on a similar intuition, we extend this method by using an extra T5 as the extrinsic model (E-T5). 
% 
An example of the template to wrap the sample into an input prompt is: ``\textless original input\textgreater, the model's prediction is \textless prediction\textgreater, is the prediction True or False? It's \textless mask\textgreater.''
% 
The probability of the ``True'' class in the calibration task is deemed as PLMs' confidence in their predictions. 
% 
The concrete manual template and verbalizer of the calibration task for each dataset are listed in Table~\ref{tab:calibration_template}.
% 

Besides, the main task model can also be directly employed to perform the calibration task. We deem this paradigm as the intrinsic one, denoted as ``I-''.
\citet{lin2022teaching} show that GPT-3~\citep{brown2020language} can be trained to output the uncertainty by words.
We adapt this method by first training the model using the main task data, and then continuing the training by using the calibration task data (I-Vanilla).
% 
However, this continual learning paradigm may result in degraded performance in the main task according to our results. 
% 
To tackle this, we propose two more practical intrinsic calibration methods through modifying the training paradigm. 
% 
Specifically, we train PLMs iteratively (I-Iter) or simultaneously (I-Simul) on the original task and the calibration task. 
The latter can be achieved due to the unified text-to-text training paradigm. 
% 
The input is the same as E-T5.
% 



% \vspace{-19pt}
%  To tackle this, I-Iterative and I-Multitask train the model iteratively or simultaneously on the original task and calibration task, respectively. 
% We implement three training paradigms for intrinsic calibration.
% The details are described in Appendix. 




% Depending on whether the calibrator is an extra model, these methods can be further divided into two categories, extrinsic and intrinsic methods, where extrinsic methods use an extra model to calibrate the predictions of the original model while intrinsic ones calibrate the model itself.
% We implement two extrinsic methods, E-MLP and E-T5, with an MLP and T5 as the backbone of the extra calibrator respectively. 
% We also implement three intrinsic methods, I-Vanilla, I-Iterative, and I-Multitask, adopting different training strategies to teach the original model to learn how to calibrate its own prediction. 
% Notably, the inputs of E-T5 and all intrinsic methods are wrapped into a calibration template and the outputs are verbalized, following the very recent ideas \citep{lin2022teaching, kadavath2022language}. 






% we train a calibrator to learn to determine whether a prediction is correct or not through the formalized calibration task. 
% To train the calibrator on the task, we relabel each sample in the validation set as \textit{True} when the original model predicts it correctly, and vice versa, as \textit{False}.

% We implement two extrinsic methods (with a prefix of "E-" in the tables), according to the backbone of the extra calibrator. 
% E-MLP uses a single-layer MLP model as the calibrator. The input of E-MLP is the concatenation of the last hidden states of the original model. 
% E-T5 copies the parameters of the original T5 model as the initialization of the calibrator. The inputs of E-T5 are wrapped into a calibration template and the output is verbalized, following the very recent ideas \citep{lin2022teaching, kadavath2022language}. 
% The templates and verbalizers used in experiments are shown in Table~. Both extrinsic methods are trained in the vanilla scheme.

% All three methods use the calibration templates and verbalizers in Table x, but they are distinct from each other in training strategies. 
% We also implement three intrinsic methods (with a prefix of "I-"), teaching the original model to learn how to calibrate its own prediction. All three methods use the calibration templates and verbalizers in Table x, but they are distinct from each other in training strategies. 
% I-Vanilla adopts the vanilla training scheme to further train the original model. Note that the final model is exactly the calibrator in E-T5. The only difference is that the input of E-T5 is the prediction of the original model, while the input of I-Vanilla is the prediction of the calibrator itself. 
% However, when learning calibration, the model might forget some knowledge of the original tasks. To tackle this, I-Iterative and I-Multitask train the model iteratively or simultaneously on the original task and calibration task, respectively. 







% \vspace{-7pt}


\subsection{Experimental Setting}
PLMs are expected to tackle out-of-distribution (OOD) samples in practice, particularly in the presence of adversarial attacks~\citep{DBLP:conf/emnlp/ChenGCQH0S22}.
% 
Thus, we experiment with both in-distribution (ID) and OOD settings. 
We consider natural language inference, sentiment analysis, and hate-speech detection tasks due to their well-established OOD datasets in NLP. 
Specifically, we choose MNLI (HANS, ANLI), Amazon (SST-5, SemEval), and Civil (Hate Speech, Implicit Hate) as the ID (OOD) datasets.
The references and detailed descriptions of chosen datasets for ID and OOD evaluation are in Appendix~\ref{sec:appendix_dataset}.
% The detailed descriptions and references are in Appendix~\ref{appendix:dataset}. 
% Note that since there is no label on the OOD datasets, we measure the calibration of each method by confidence and entropy. 
% A well-calibrated model should be unconfident in the task-irrelevant inputs, with low confidence and high entropy.

% Moreover, since we need to train a model on calibration tasks for learnable methods, it is necessary to figure out how the dataset size and model scale affect the calibration. 
% Hence, we explore the emergent calibration of learnable methods by training the calibrators on validation datasets of different sizes and employing models of different scales as backbones. 
% Specifically, we consider Amazon and T5. We sample the original validation dataset used in previous experiments to construct the small- and middle-size validation set. For experiments on the dataset size, we adopt T5-base as the backbone model and train it using different devsets. For experiments on the model scale, we train T5-small/base/large models using the middle-size devset.







\subsection{Experimental Results}
\label{sec:standard}
% \looseness=-1
The results are listed in Table~\ref{tab:t5-shift} (T5) and Table~\ref{tab:roberta-shift} (RoBERTa). 
We summarize the overall conclusions as follows:
All calibration methods have negligible influence on PLMs' performance in the ID and OOD settings except I-Vanilla.
However, PLMs are significantly less calibrated under considered distribution shifts, especially on challenging datasets due to the severe mismatch between performance and confidence. 
For example, the vanilla T5 achieves only 30.53\% accuracy on ANLI, but its average confidence is up to 93.77\%. 
For ID evaluation, we observe lower ECE, consistent with \citet{DBLP:conf/emnlp/DesaiD20}.
However, the conclusion that PLMs are calibrated on ID data~\citep{DBLP:conf/emnlp/DesaiD20} is questionable given our answer to the first question (see Sec.~\ref{sec:empirical_study}).
% we consider the conclusion that PLMs are calibrated on ID data.
The low ECE can be attributed to their high performance on ID datasets and consistently assigning high confidence scores to their predictions. 
% 
We further show the conclusion that PLMs calibration degrades under distribution shifts is one-sided and heavily depends on the evaluation datasets chosen in Appendix \ref{sec:further_dis}.
% conduct further analysis on the PLMs calibration degradation under distribution shifts in Sec.~\ref{sec:further_dis}.


% given the high CErr$_{neg}$, the previous conclusion that PLMs are calibrated on in-distribution data~\citep{DBLP:conf/emnlp/DesaiD20} should be reconsidered. 
% Again, the high CErr$_{neg}$ indicates that PLMs don't have clear estimations of predictive uncertainty.




% A most extreme case is a model that knows nothing about calibration but just learns to be very confident on its prediction in the learning process. 
% Then if this model can make correct predictions on most testing cases (like modern PLMs), it will obtain high accuracy along with low ECE.  
% We show supporting cases when measured on challenging datasets in the next section.


% \looseness=-1
\textbf{Unlearnable methods.} 
We summarize the findings as follows:
(1) Data augmentation and model ensemble don't bring substantial benefits to PLMs calibration, considering the three calibration metrics spanning all evaluation datasets and two PLMs.
The reason lies in their inability to relieve the overconfident issue, resulting in the same Cerr$_{neg}$ with the vanilla fine-tuning;
(2) TS achieves overall better ECE, maintaining a strong baseline method, with LS being the second effective method for the unlearnable category.
This is consistent with previous empirical studies~\citep{DBLP:conf/cvpr/NixonDZJT19}.
However, we can observe almost the same amount of increase in CErr$_{pos}$ with the decrease in CErr$_{neg}$. 
The reason is that these two methods directly impose confidence regularization on predictions, which don't actually make PLMs have clear confidence estimations.






% However, though employing TS and LS improves PLMs calibration considering ECE and CErr$_{neg}$, blindly imposing confidence regularization increases CErr$_{pos}$.
% In practice, this is also undesirable because we may reject correct predictions due to their relatively low confidence. 
% Thus, these two methods don't actually improve model calibration, enabling models to have reasonable confidence in their predictions. 
% Instead, they are just good players in the ``calibration game'' with ECE as the referee. 



\input{tab/emergent_devset_size.tex}

\looseness=-1
\textbf{Learnable methods.}
Compared to unlearnable methods, learnable ones significantly mitigate the overconfidence issue, reflected in the sharp decrease in CErr$_{neg}$, indicating that learnable methods output very low confidence in wrong predictions.
But we also observe that learnable methods lower the confidence in correct predictions, resulting in increasing CErr$_{pos}$ and ECE. 
However, we highlight two observations indicating that learnable methods essentially teach models to have clearer confidence estimations, instead of roughly reducing the confidence like LS:  
(1) Compared to the vanilla version, the increase in CErr$_{pos}$ is significantly lower than the decrease in CErr$_{neg}$, especially on ID samples; 
(2) Learnable methods give obviously lower confidence in OOD samples, and the average confidence drop is highly relevant to the performance drop under distribution shifts. 
Thus, the low confidence and relatively higher CErr$_{pos}$ and ECE on OOD samples may be reasonable.
% accepted since PLMs are unfamiliar with them. 


% (1) The average confidence scores on OOD samples are significantly lower than in-distribution samples; 
% (2) There is a sharp decrease in

% This is accepted when dealing with out-of-distribution data that models may be unfamiliar with; 
% (3) Given the trade-off, this can be application-specific to decide whether to adopt learnable calibration methods. For example, if working on the scenarios when accepting wrong predictions will cause significant damage, then the learnable methods are recommended.

% (2) The relative less confidence on correct predictions may be partially explained by some supporting evidence in samples. Namely, although making correct predictions,  models can have some uncertainty;



Further, we give a detailed analysis of extrinsic and intrinsic learnable methods and also compare our extended calibration methods with previous methods:
% Then we compare the extrinsic and intrinsic methods:
(1) For extrinsic methods, the extended E-T5 exhibits significantly better calibration performance compared to the adapted E-MLP considering the mitigation of the overconfidence issue.
The essential difference mainly lies in the extrinsic model for the calibration task.
We find that using the larger capacity model as the extrinsic calibrator shows the same trend with shifting from the vanilla fine-tuning to learnable methods. 
We further study this scaling effect in Sec.~\ref{sec:emergent};
(2) For intrinsic methods, the three different training paradigms don't show substantial differences considering the calibration performance, and none of them consistently achieves the best performance on all datasets.
As a comparison, our methods (I-Iter and I-Simul) address the degraded performance issue of I-Vanilla and make the main task performance match with the vanilla fine-tuning;
% But we identify great potential in designing new training paradigms to better learn the calibration task.
% And future work is needed to explore the relationship between the calibration task and the main task when modeled as a multi-task learning problem;
(3) Interestingly, there doesn't exist a substantial difference between the extrinsic E-T5 method and other intrinsic methods, given the same base architecture (e.g., T5). 
% Note that the base architecture is the same, indicating the same model capacity. 
This finding leads us to reconsider the conclusion in \citet{lin2022teaching} that PLMs can be trained to give their uncertainty by words. 
Given the comparable performance between intrinsic and extrinsic methods, we provide an extension to this conclusion.
We identify that the success of this paradigm essentially lies in the learnable attribute of the calibration task, instead of the self-checking process of PLMs.
Namely, the findings in previous work may not only be attributed to the capability of PLMs but also the ”learnable” property of the calibration task. 



% % \paragraph{Learnable Methods.} We summarize the results as follows: 
% \begin{itemize} [topsep=1pt, partopsep=1pt, leftmargin=12pt, itemsep=0pt]
% \end{itemize}


% \paragraph{Summary.} We show the feasibility to formalize the model calibration into a learnable task and observe great potential in learnable calibration methods compared to unlearnable ones. 
% But there still exists some trade-offs when adopting learnable methods, such as the decrease in confidence in correct predictions. 






\subsection{Emergent Calibration}
% \looseness=-1
\label{sec:emergent}
In Sec.~\ref{sec:standard}, we identify the potential in learnable methods. 
However, a detailed exploration of learnable calibration methods is lacking. 
We conduct experiments to study the influence of two important factors, namely the dataset size and the model scale for the calibration task, on PLMs calibration.
% We study the influence of increasing dataset size and model scale for learnable calibration methods. 
Note that the model scale in this section considers the model adopted for the calibration task, instead of the main task.
  
\textbf{Dataset size.}
% \looseness=-1
Table~\ref{tab:emergent_dev_size} shows the results of different sizes of the calibration dataset. 
Two basic findings are:
(1) The five learnable methods show a consistent trend when increasing the dataset size, indicating that the essence of these methods is the same;
(2) The size of datasets for training the calibration task doesn't have a substantial influence on PLMs performance on the main task.

% \looseness=-1
Beyond these, we observe that there is a sharp difference in calibration performance when increasing the dataset size from small to middle. The trend is overall consistent with the one observed when shifting from vanilla fine-tuning to learnable calibration methods. 
The trend can be summarized as:
(1) For ID samples, we can observe a sharp decrease in CErr$_{neg}$ with relatively less negative influence on ECE and CErr$_{pos}$;
(2) For OOD samples, the CErr$_{pos}$ and ECE increase significantly along with increasing the dataset size. 
However, given the arguments in Sec.~\ref{sec:standard}, we identify that PLMs' calibration performance improves when trained on larger calibration datasets. 
Besides, we don't observe further improvement in calibration performance when increasing the dataset size from middle to large. 
This is consistent with normal task training, where increasing the dataset size doesn't increase performance after a critical point.


% Again, we argue the reasonability of being unconfident in OOD samples, even though the predictions may turn out to be correct; 
% (4) Given the comparable performance between middle and large dataset sizes and the sharp difference in calibration performance between the small size and others, we hypothesize that there exists a critical point in the dataset scaling process.
% Before this point, PLMs show emergent calibration ability.
% % since Conf, ECE, CErr$_{pos}$, and CErr$_{neg}$ show similar trends consistent with the ones when shifting 
% After this point, introducing more samples doesn't bring substantial difference to PLMs calibration.
% The existence of the critical point 




\textbf{Model scale.}
\looseness=-1
Table~\ref{tab:emergent_scale} shows the results of various model scales. 
Two basic findings are:
(1) The five learnable methods still show a consistent trend when scaling larger; 
(2) We observe a consistent confidence increase when scaling larger, which is similar to the trend observed in Sec.~\ref{sec:empirical_study}, where increasing capacity makes PLMs more confident. 

\looseness=-1
Surprisingly, although the confidence continues to increase, for ID samples, we observe a consistent decrease in CErr$_{pos}$ with neglectable influence on ECE and CErr$_{neg}$ when scaling larger.
% Namely, model learns to become confident on their correct predictions and vice versa;  
Note that the dataset for the calibration task is collected from ID.
Thus, if provided enough ID samples for the calibration task training, scaling larger enables models to better learn the calibration task, ensuring better calibration performance on ID samples.
For OOD samples, we don't observe a consistent trend due to the influence of various factors.
% 
Specifically, when using out-of-the-box to tackle OOD samples, the  problem of distribution shifts appears in the introduced calibration task.
Whether scaling the calibration-task model larger improves calibration performance under distribution shifts is determined by many factors (e.g., the dataset difficulty, the overconfidence issue in the calibration task).
We leave it for future exploration.
% we still observe the consistent decrease in ECE, CErr$_{pos}$ when scaling larger. 
% However, the CErr$_{neg}$ shows a tendency to decrease and then increase. 
% Note that 
% Thus, the conclusions are:
% (1) If provided the 
% (2) 


% Given our empirical study in Sec~\ref{sec:empirical_study}, we hypothesize that there also exists the calibration problem in the calibration task. 
% Namely, model may be overconfident in their predictions of whether the answer is correct.
% Thus, keep scaling is not always better under distribution shifts. 
% and it's important to find an appropriate model scale. This conclusions is consistent with Sec.~\ref{sec:increasing_scale}.










% PLMs' relative calibration performance on ID and OOD samples relies on the dataset difficulty


% (3) Across all methods, the confidences on random tokens is higher than the ones on plain text.  the counter-intuitive results.



% \input{tab/entropy_t5.tex}










==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/conclusion.tex <==
\section{Conclusion}
% \looseness=-1
We take a close look into PLMs calibration, motivating to answer two central questions:
% 
(1) Do PLMs learn to become calibrated in the training process? 
(2) How effective are existing calibration methods?
We present a comprehensive empirical study, including the analysis of various decisive factors and concrete calibration methods.
Besides the findings that support existing conclusions, we also provide extensions or contradictory arguments to some established conclusions. 
% We conduct an empirical study, motivating to answer two questions: 
% 



\section*{Limitations and Future Work}
We identify two limitations in our work that necessitate further investigation and improvement.
% 
First, only empirical results are presented in our work. 
% 
A theoretical understanding of PLMs calibration is still lacking.
% 
Going forward, we are motivated to investigate this problem from the standpoint of feature learning.
% 
We see great potential in unifying several problems in AI safety~\citep{DBLP:journals/corr/abs-2104-14235} from a feature-learning perspective, including spurious correlations~\citep{DBLP:conf/acl/GuWCL19, DBLP:conf/naacl/WangSY022}, robustness~\citep{DBLP:journals/corr/abs-2110-15317, DBLP:conf/acl/0002PTK22}, backdoor learning~\citep{DBLP:conf/qrs/ShengHLC22, DBLP:conf/nips/CuiYHCLS22}, and calibration~\citep{DBLP:conf/emnlp/UlmerFH22}. 
Second, we propose three simple extended calibration methods based on existing ones. 
% 
In our experiments, we evaluate the calibration performance of existing and our calibration methods.
% 
We make an assumption that we have a large held-out validation set that can be employed as the training dataset for the calibration task.
% 
We demonstrate the effectiveness of learnable calibration methods in this ideal situation.
% 
However, in practice, we need to make the decision about how to allocate the data for the main task and the calibration task given limited training samples.
% 
 


% We plan to study a more practical scenario when we have a certain number of training samples and propose a training framework that can make the most of training samples for both the main task and the calibration task. 








% In the future, we plan to explore more about learnable calibration methods.
% In this paper, we show the potential in them, especially when adopting large capacity models and provided enough ID calibration training samples. 
% A detailed analysis about the calibration task is needed, including the acquisition of informative training data, the training paradigm, and its relationship with the original task.








%  \textbf{Learnable calibration method.} In this paper, in learnable calibration methods, rather than shallow classifiers. 
% Future works can better explore the calibration task, including the 

% Our empirical study includes (1) a fine-grained analysis of six dimensions for their influence on the calibration performance, and (2) a detailed evaluation of calibration methods in both in-distribution and OOD settings.




% In the first stage analysis, we find a consistent trend that calibration performance is highly relevant with PLMs' fitness on training samples. 
% And the fitness is dynamically influenced by the six identified dimensions. 
% Based on the empirical findings, we 



% reexamination of established conclusions, a fine-grained analysis of our identified four factors that have significant influence on model calibration, and calibration methods in in-distribution and out-of-distribution settings. 
% We draw a bunch of findings throughout the three parts in our empirical study. 
% Some of them are consistent with previous works. 
% But we have also come to new conclusions, some at odds with previous findings. 

% \paragraph{Future Works.}
% (1) \textbf{Calibration metrics.} 
% We show that measuring ECE can only present one single face of model calibration, resulting in incomprehensive understanding of calibration. 
% New informative metrics can be designed to evaluate model calibration from different perspectives. 
% (2) \textbf{Calibration evaluation.}
% We show that models' calibration performance is sensitive to training steps, the choice of datasets, and the model capacity. 
% Thus, how to conduct more rigorous evaluations and comparisons of model calibration need to be further explored. 
% % {.\yang{may to separate into two parts, measure and analysis}} more precise and comprehensive evaluation (variance due to training steps et al, not good metrics).
% (3) 
 


% Different from previous coarse-grained analysis that focus on some specific techniques (e.g., pretraining, model architecture), we conduct an empirical study considering five dimensions in the training process that have significant influence on model calibration. 
% Specifically, we consider available training samples, training steps, the number of tunable parameters, intervention of calibration methods, and distribution shifts.
% Then we reexamine two established conclusions, and draw some conclusions that are inconsistent with previous works. 
% We give a summary of our empirical study in the discussion section, outlining four important factors impacting on model calibration. 




==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/discussion.tex <==
% \section{Discussion}


% \begin{wrapfigure}{r}{0.3\textwidth}
% \begin{center}
%     % \vspace{-40pt}
%     \includegraphics[width=\linewidth]{figures/demons.pdf}
% \end{center}
%     \caption{caption}
%     \label{fig:demons}
% \end{wrapfigure}


% In this section, we first summarize our empirical study into a unified framework to understand model calibration. 
% Then we discuss the connection and conflict between our study and previous findings. 
% Finally, we propose potential future directions in model calibration. 

% \paragraph{Summary of Our Study. }

% In previous works, empirical studies on model calibration have been conducted from different perspectives, including the influence of model architectures~\citep{DBLP:conf/cvpr/NixonDZJT19}, the in-distribution or out-of-distribution dataset~\citep{DBLP:conf/emnlp/KongJZLZZ20}, model scale~\citep{srivastava2022beyond}, pretraining~\citep{hendrycks2019using}, and so on. 
% In our study, we take a fine-grained look into model calibration. 
% Given our empirical results, we now propose a unified understanding of model calibration, outlining five deterministic factors: (1) Model capacity (model scale, the number of tunable parameters, pretraining); (2) Available training signals (shot number); (3) Fitness on training samples (training step); (4) Dataset difficulty; (5) Confidence regularization (calibration method).  
% The notations in parentheses highlight the choices that impact the selected factors. 
% These factors have large influence on model performance and corresponding confidence, thus determining calibration.  
% We give a sketch in Figure~\ref{fig:demons} and summarize our empirical findings: 
% \begin{itemize} [topsep=1pt, partopsep=1pt, leftmargin=12pt, itemsep=-2pt]
%     \item As continually fitted on a dataset, (almost) all DNNs will gain higher performance and confidence in the early stage. 
%     While the performance may saturate after a certain step, model confidence will continue to increase (almost close to 100) when trained longer.
%     Thus, training longer increase the calibration error (a-b). 
%     \item Model capacity affects both confidence and performance. 
%     Thus, when the performance cannot be further improved by increasing model capacity due to the inborn difficulty of the dataset (discussed later), more capacity only brings a more over-confident model, which has negative influence on model calibration. 
    
%     \item Available training signals affect in the same way as model capacity, although in a mild way.
%     Again, keep increasing training signals after the time model performance saturates only brings a more over-confident model. 
    
    
%     \item The dataset difficulty is decisive for model performance, while has less influence on confidence. 
%     For example, DNNs still gain over 90 average confidence score on ANLI with near 25 accuracy score.
%     In the era of DNNs, higher difficulty translates to lower b and nearly constant a in Figure~\ref{fig:demons}, which significantly increases the gap and results in high calibration error. 
    
    
%     \item As observed in our empirical study, only calibration methods that function as confidence regularization can take effect in model calibration. 
%     It can be translated to roughly reducing \textbf{a} in Figure~\ref{fig:demons}, exploiting the weakness and learning behavior of modern DNNs. 
%     However, models don't learn to be calibrated when intervened in this process, since confidence regularization is unlearnable. 
    
    
    
    
    
% \end{itemize}














% \paragraph{The Connection and Conflict with Previous Findings.}
% In our empirical study, we also consider the ECE score following previous works~\citep{DBLP:conf/cvpr/NixonDZJT19, DBLP:conf/emnlp/KongJZLZZ20} since it's a direct measure of model calibration.
% We show consistent experimental results in some settings. 
% For example, when increasing capacity (e.g., scaling larger, more tunable parameters) brings substantial improvement on model performance, we can observe a clear decrease in ECE. 
% Besides, we evaluate on in-distribution and out-of distribution settings, showing consistent results that models tend to be less calibrated under distribution shifts.
% Across almost all settings and datasets, we quantitatively show the problem of unmatched confidence and accuracy, which has been revealed in previous works. 
% The highlight in this paper is a fine-grained multi-dimensional analysis.
% Different from previous works that conduct an one-pass evaluation, we decompose the learning pipeline, covering many aspects in the training process. Thus, new and conflict findings emerge: 
% (1) Pretraining, scaling, and larger capacity doesn't guarantee a more calibrated model; 
% (2) More proficient on the dataset may bring negative effect on model calibration. 


% \paragraph{Future Works.}
% (1) \textbf{Calibration Metrics.} 
% We show that measuring ECE can only present one single face of model calibration, resulting in incomprehensive understanding of calibration. 
% New informative metrics can be designed to evaluate model calibration from different perspectives. 
% (2) \textbf{Calibration Evaluation.}
% We show that models' calibration performance is sensitive to training steps, the choice of datasets, and the model capacity. 
% Thus, how to conduct more rigorous evaluations and comparisons of model calibration need to be further explored. 
% % {.\yang{may to separate into two parts, measure and analysis}} more precise and comprehensive evaluation (variance due to training steps et al, not good metrics).
% (3) \textbf{Learnable Calibration Method.} In this paper, we show potential in learnable calibration methods, especially when adopting large capacity models rather than shallow classifiers. 
% Future works can better explore the calibration task, including the acquisition of informative training data, the training paradigm, and its relationship with the original task. 


% % (3) \textbf{Understanding.} Theoretical understanding of the whole learning process on model calibration. 








==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/empirical_experiments.tex <==


\input{fig_latex/avai_train_samples_t5}
\input{fig_latex/dynamics_t5}




\section{\looseness=-1 Do PLMs Learn to Become Calibrated?}
\label{sec:empirical_study}
% In this section, we motivate to answer: Does PLMs learn to become calibrated in the training process? 
% We first describe the experimental settings, and then summarize the conclusions. 





\subsection{Experimental Setting}
\looseness=-1
For model architectures, we choose RoBERTa-base~\citep{liu2019roberta} and T5-base~\citep{DBLP:journals/jmlr/RaffelSRLNMZLL20}, since they represent two classic types of PLMs, namely encoder-only and encoder-decoder models.
We experiment with four representative tasks in NLP, including sentiment analysis, natural language inference, news classification, and topic classification.
For datasets, we choose SST-2~\citep{DBLP:conf/emnlp/SocherPWCMNP13}, MNLI~\citep{DBLP:conf/naacl/WilliamsNB18}, AG-News~\citep{DBLP:conf/nips/ZhangZL15}, and Yahoo~\citep{DBLP:conf/nips/ZhangZL15} respectively. 
We employ the prompt-based learning paradigm~\citep{liu2021pre} since its superior performance compared to traditional fine-tuning, especially in the few-shot setting.
Specifically, we inherit the masked language modeling task in the pre-training stage and use templates to wrap samples into prompts.
% 
We fine-tune the whole PLMs to fill in the [mask] position in the prompt. 
The manual template and verbalizer for each dataset are listed in Appendix~\ref{sec:appendix_dataset}. 


\input{fig_latex/params_t5_adapter}
\input{fig_latex/scale_t5}
\input{fig_latex/pretrain_t5}

% In fact, we can attribute the influence to the increase in models capacities.
% Besides, we also identify three other factors that may affect model calibration and are often overlooked in previous works, named available training signals, fitness on training samples, and dataset difficulty. 
\subsection{Experimental Results}
\looseness=-1
We conduct a fine-grained control study to explore the influence of six factors, 
including dataset difficulty, available training samples (Fig.\ref{fig:kshots-t5}), training steps (Fig.\ref{fig:dynamics-t5}), number of tunable parameters (Fig.\ref{fig:adapter-t5} and Fig.\ref{fig:soft_prompt-t5}), pretraining (Fig.\ref{fig:pretrain}), and model scale (Fig.\ref{fig:scale-t5}). 
% All six factors have substantial influence on PLMs' fitness on the training distribution.
Due to space limits, we show the corresponding results of RoBERTa and results of T5 on AG-News in Appendix~\ref{sec:appendix_additional_first}.
We summarize the overall conclusions and leave the detailed experimental settings and findings in Appendix~\ref{sec:appendix_additional_first}. 




\looseness=-1
We note that all six factors dynamically influence PLMs' fitness on the training distribution, which we identify as the decisive factor of PLMs' calibration performance. 
% We draw the conclusion for the first question: PLMs' calibration performance is highly determined by their fitness on the training distribution.
% All six factors dynamically influence PLMs' fitness.
% For example, increasing the number of tunable parameters or training longer both make PLMs more fitted.
We observe an overall consistent change in calibration performance across six factors, resulting in two PLMs' states (see Fig.\ref{fig:hello}) in training:


\looseness=-1
\textbf{Under-fitted state.}
In this state, PLMs' performance and confidence increase at different speeds when more fitted on the training distribution.
The ECE score fluctuates during this process.
In principle, miscalibration is due to the mismatch between performance and confidence.
However, we look closely into some critical points where ECE changes sharply (e.g., Fig.\ref{fig:kshots-t5}), and empirically find that the increase or decrease in ECE can be estimated by comparing the increasing rates of PLMs' performance and confidence.
We observe that a larger (smaller) increasing rate in performance reduces (increases) ECE.
Thus, high ECE can be partially attributed to PLMs' relatively rapid growth in confidence with performance lagging behind. 
% Typically, miscalibration is due to the mismatch between two trends, where



\textbf{Over-fitted state.}
In this state, PLMs' performance doesn't have a substantial difference due to their generalization ability~\citep{zhang2021understanding}. 
However, PLMs' confidence continues to increase in this state, resulting in increasing ECE.
% 
This is especially obvious when more training steps and tunable parameters are introduced (see Fig.\ref{fig:dynamics-t5} and Fig.\ref{fig:adapter-t5}). 
% 
Thus, being more fitted on the training distribution may bring a negative effect on PLMs calibration. 
In addition, due to the increase of ECE in this state, the evaluation of calibration performance may be sensitive to the training paradigm.
This indicates that previous conclusions drawn from empirical studies should be carefully examined since the training paradigms may be different in model architectures and calibration methods.
% 

\looseness=-1
Given the two states observed, we conclude that \textbf{PLMs don't learn to become calibrated in training, evidenced by the continually increasing confidence in predictions, no matter correct or not, in the fitting process.} 
% 
Specifically, this results in two miscalibration behaviors:
(1) Increasing ECE in the over-fitted state;
(2) The consistent increase in CErr$_{neg}$ throughout the whole training process. This is an undesirable property in practice since users may accept wrong predictions due to their high confidence, and indicates that PLMs mostly don't know ``what they don't know''. 




\looseness=-1  
We highlight two of the considered factors, namely pretraining and model scales (Fig.\ref{fig:scale-t5} and Fig.\ref{fig:pretrain}), which are examined in previous work.
Our findings present some contradictory views with the established conclusions:
(1) Larger PLMs show better calibration~\citep{srivastava2022beyond};
(2) Pretraining improves model calibration~\citep{hendrycks2019using}.
Actually, scaling larger and employing pretraining are both strategies to increase PLMs capacity, making them more fitted on the training distribution.
Our general conclusion can also be applied. 
We highlight two observations: 
(1) Essentially, the influence of scaling larger and pretraining on PLMs calibration is dynamically determined by the relative increase in performance and confidence, which is highly relevant to the chosen evaluation datasets.
For example, the original scaling experiments are conducted on BIG-bench~\citep{srivastava2022beyond}, in which the performance is far from saturation and increasing the model scale brings substantial improvement to PLMs performance.
This shows consistency with the identified under-fitted state.
However, when the performance score saturates on evaluation datasets given the certain scale of PLM, scaling larger will only bring up confidence. 
This results in increasing ECE due to the mismatch between two trends (e.g., T5 and RoBERTa on Yahoo);
(2) Scaling larger and employing pretraining consistently bring CErr$_{neg}$ higher.
This indicates that these two strategies don't enable PLMs to learn to become calibrated in the training process.



% \vspace{-5pt}



% The ECE is determined by the racing game between models' performance and confidence. 
% Thus, the ``scaling improves calibration'' conclusion depends on datasets and models. 

% Our results support this conclusion in some cases.
% We observe that ECE decreases when larger capacity brings substantial improvement to models' performance (e.g., T5 on SST-2 and MNLI). 
% However, when the performance reaches a plateau value, increasing capacity only boosts models' confidence (e.g., T5 on Yahoo, RoBERTa on MNLI and Yahoo). 
% In this case, the ECE increases when the model scale keeps increasing.


% \end{itemize}




% 
% \vspace{10pt}


==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/exp_setting.tex <==
\section{Evaluation Metrics} 
\label{sec:exp_setting}




% \paragraph{Evaluation metrics.}
% \looseness=-1
For basic evaluation, we report accuracy (Acc) and average confidence score (Conf) on the testing set.
For calibration evaluation, we report ECE using equal-mass binning and 100 bins following \citet{DBLP:conf/nips/MindererDRHZHTL21}.
Besides, we provide an application-driven perspective to evaluate model calibration, aiming to quantify two unsatisfied scenarios due to miscalibration in practice:
(1) Correct predictions (positive) are rejected due to low confidence; 
(2) Wrong predictions (negative) are accepted due to high confidence. 
Specifically, we consider the average confidence in correct predictions $\textbf{Conf}_{pos}$ and wrong predictions $\textbf{Conf}_{neg}$ respectively.
For unified comparison, we report two calibration error (CErr) cases, $\text{CErr}_{pos}=1-\text{Conf}_{pos}$ and $\text{CErr}_{neg}=\text{Conf}_{neg}$. 
In principle, we expect calibrated models to have both low CErr$_{pos}$ and CErr$_{neg}$, indicating that they reasonably assign high confidence in correction predictions and low confidence in wrong predictions. 




% To formalize, we denote the testing case as $(x, y)$ and model prediction as $\hat{y}$.
% We compute the calibration error on positive and negative cases separately:
% \begin{equation}
% \begin{split}
% &\text{CErr}_{pos} = \frac{1}{n_{pos}}\sum_{i=1}^{n_{pos}}{(1-\text{Conf}(x_i, \hat{y}_i))}, \quad  \hat{y}_i = y_i,   \\
% &\text{CErr}_{neg} = \frac{1}{n_{neg}}\sum_{i=1}^{n_{neg}}{\text{Conf}(x_i, \hat{y_i})}, \quad \hat{y_i} \neq y_i,
% \\
% \end{split}
% \end{equation}
% where Conf$(x,\hat{y})$ is the predictive probability of prediction $\hat{y}$ on sample x.
% We note that this application-driven perspective motivates the same formula mentioned in \citet{si2022revisiting}. 
% They take a step further to compute the macro average of CErr$_{pos}$ and CErr$_{neg}$. 
% However, we show that measuring them separately provides more accurate and fine-grained results. 








==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/fig_latex/additional_t5.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
    \centering
    \includegraphics[trim=0 0 0 0, clip, width=\textwidth]{figures/shots-t5-agnews.pdf}
     \label{fig:kshots-t5-agnews}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[trim=0 0 0 0, clip,width=\textwidth]{figures/dynamics-t5-agnews.pdf}
     \label{fig:dynamics-t5-agnews}
    \end{subfigure}     
     \begin{subfigure}[b]{0.322\textwidth}
     \includegraphics[trim=0 0 0 0, clip,width=\textwidth]{figures/delta-adapter-t5-agnews.pdf}
     \label{fig:adapter-t5-agnews}
     \end{subfigure}

    \vspace{-7pt}
     \begin{subfigure}[b]{0.6\textwidth}
         \centering
         \includegraphics[trim=0 0 0 0, clip, width=\textwidth]{figures/legend.pdf}
        %  \label{fig:kshots-t5-yahoo}
    % \vspace{18pt}
     \end{subfigure}
     
     \vspace{-6pt}
     \caption{Additional results of T5 on AG-News including the influence of the number of training samples, training steps, and the tunable parameters number.}
     % \vspace{-10pt}
     \label{fig:t5-agnews}
\end{figure*}




\begin{figure*}
\centering
    \begin{minipage}[b]{0.46\textwidth}
        \includegraphics[trim=0 0 0 0 , clip,width=0.93\textwidth]{figures/scale-t5-agnews.pdf}
        \caption{Additional results of different PLMs scales with T5 on AG-News.}
         \label{fig:scale-t5-agnews}
    \end{minipage}
    \quad
    \begin{minipage}[b]{0.43\textwidth}
        \includegraphics[width=\textwidth]{figures/pretrain-t5-agnews.pdf}
        \caption{Additional results of the pretraining influence with T5 on AG-News.}
         \label{fig:pretrain-t5-agnews}
    \end{minipage}
\end{figure*}



\begin{figure*}[!h]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim=0 0 0 0, clip, width=\textwidth]{figures/soft_prompt-t5-sst2.pdf}
         \label{fig:soft_prompt-t5-sst2}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim=0 0 0 0, clip,width=\textwidth]{figures/soft_prompt-t5-mnli.pdf}
         \label{fig:soft_prompt-t5-mnli}
     \end{subfigure}

     \vspace{-5pt}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim=0 0 0 10, clip,width=\textwidth]{figures/soft_prompt-t5-yahoo_answers_topics.pdf}
         \label{fig:soft_prompt-t5-yahoo}
     \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim=0 0 0 10, clip,width=\textwidth]{figures/soft_prompt-t5-agnews.pdf}
         \label{fig:soft_prompt-t5-agnews}
     \end{subfigure}

     \vspace{-7pt}
     \begin{subfigure}[b]{0.6\textwidth}
         \centering
         \includegraphics[trim=0 0 0 10, clip, width=\textwidth]{figures/legend.pdf}
        %  \label{fig:kshots-t5-yahoo}
    % \vspace{18pt}
     \end{subfigure}
        
    \vspace{-5pt}
    \caption{Results of tunable parameters with T5 (Soft-prompt).}
    % \vspace{1pt}
    \label{fig:soft_prompt-t5}
    \vspace{-5pt}
\end{figure*}

==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/fig_latex/avai_train_samples_roberta.tex <==
\begin{figure*}[t]
     \centering
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/shots-roberta-sst2.pdf}
         \label{fig:kshots-roberta-sst2}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/shots-roberta-mnli.pdf}
         \label{fig:kshots-roberta-mnli}
     \end{subfigure}
    %  \hfill
    
    \vspace{-5pt}
    \centering
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/shots-roberta-agnews.pdf}
         \label{fig:kshots-roberta-agnews}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[trim=0 0 0 0, clip, width=\textwidth]{figures/shots-roberta-yahoo_answers_topics.pdf}
         \label{fig:kshots-roberta-yahoo}
     \end{subfigure}

     \vspace{-15pt}
     \begin{subfigure}[b]{0.6\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/legend.pdf}
        %  \label{fig:kshots-t5-yahoo}
     \end{subfigure}
     
    \vspace{-5pt}
    \caption{Results of available training samples with RoBERTa.}
    \label{fig:kshots-roberta}
    % \vspace{-20pt}
\end{figure*}

==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/fig_latex/avai_train_samples_t5.tex <==

% \begin{wrapfigure}{r}{0.66\textwidth}
    
%      \centering
%      \begin{subfigure}[b]{0.32\textwidth}
%          \centering
%          \includegraphics[trim=0 10 0 0, clip, width=\textwidth]{figures/kshots-t5-sst2.pdf}
%          \label{fig:kshots-t5-sst2}
%      \end{subfigure}
%     %  \hfill
%      \begin{subfigure}[b]{0.32\textwidth}
%          \centering
%          \includegraphics[trim=0 10 0 0, clip,width=\textwidth]{figures/kshots-t5-mnli.pdf}
%          \label{fig:kshots-t5-mnli}
%      \end{subfigure}
%     %  \hfill
%     \vspace{-10pt}
    
%     \centering
%      \begin{subfigure}[b]{0.32\textwidth}
%          \centering
%          \includegraphics[trim=0 10 0 0, clip,width=\textwidth]{figures/kshots-t5-agnews.pdf}
%          \label{fig:kshots-t5-agnews}
%      \end{subfigure}
%     %  \hfill
%      \begin{subfigure}[b]{0.32\textwidth}
%          \centering
%          \includegraphics[trim=0 10 0 0, clip, width=\textwidth]{figures/kshots-t5-yahoo_answers_topics.pdf}
%          \label{fig:kshots-t5-yahoo}
%      \end{subfigure}
%      \vspace{-5.5pt}
%      \begin{subfigure}[b]{0.6\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/legend.pdf}
%         %  \label{fig:kshots-t5-yahoo}
%      \end{subfigure}
       
%         \caption{Results on available training samples with T5.}
%         \label{fig:kshots-t5}
% \end{wrapfigure}


\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim=0 10 0 0, clip, width=\textwidth]{figures/shots-t5-sst2.pdf}
         \label{fig:kshots-t5-sst2}
     \end{subfigure}  
    \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim=0 10 0 0, clip,width=\textwidth]{figures/shots-t5-mnli.pdf}
         \label{fig:kshots-t5-mnli}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim=0 10 0 0, clip, width=\textwidth]{figures/shots-t5-yahoo_answers_topics.pdf}
         \label{fig:kshots-t5-yahoo}
     \end{subfigure}
     
     \vspace{-11pt}
     \begin{subfigure}[b]{0.6\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/legend.pdf}
        %  \label{fig:kshots-t5-yahoo}
     \end{subfigure}
         \vspace{-5pt}
        \caption{Results of available training samples with T5.}
        \label{fig:kshots-t5}
\end{figure*}


==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/fig_latex/dynamics_roberta.tex <==
\begin{figure*}[!h]
     \centering
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/dynamics-roberta-sst2.pdf}
         \label{fig:dynamics-roberta-sst2}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/dynamics-roberta-mnli.pdf}
         \label{fig:dynamics-roberta-mnli}
     \end{subfigure}
    %  \hfill
    
    \vspace{-5pt}
    \centering
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/dynamics-roberta-agnews.pdf}
         \label{fig:dynamics-roberta-agnews}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/dynamics-roberta-yahoo_answers_topics.pdf}
         \label{fig:dynamics-roberta-yahoo}
     \end{subfigure}

     \vspace{-18pt}
     \begin{subfigure}[b]{0.6\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/legend.pdf}
        %  \label{fig:kshots-t5-yahoo}
     \end{subfigure}
     
    \vspace{-5pt}
    \caption{Results of training steps with RoBERTa.}
    \label{fig:dynamics-roberta}
\end{figure*}

==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/fig_latex/dynamics_t5.tex <==

\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim=0 0 0 0, clip,width=\textwidth]{figures/dynamics-t5-sst2.pdf}
         \label{fig:dynamics-t5-sst2}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim=0 0 0 0, clip,width=\textwidth]{figures/dynamics-t5-mnli.pdf}
         \label{fig:dynamics-t5-mnli}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim=0 0 0 10, clip,width=\textwidth]{figures/dynamics-t5-yahoo_answers_topics.pdf}
         \label{fig:dynamics-t5-yahoo}
     \end{subfigure}
        % \vspace{-10pt}
        
    \vspace{-13pt}
        
     \begin{subfigure}[b]{0.6\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/legend.pdf}
        %  \label{fig:dynamics-t5-yahoo}
     \end{subfigure}
        % \vspace{-6pt}
        \vspace{-5pt}
        \caption{Results of training steps with T5.}
        % \vspace{-5pt}
        \label{fig:dynamics-t5}
\end{figure*}


==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/fig_latex/params_roberta.tex <==
\begin{figure*}[t]
     \centering
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/delta-adapter-roberta-sst2.pdf}
         \label{fig:parameter-roberta-sst2}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/delta-adapter-roberta-mnli.pdf}
         \label{fig:parameter-roberta-mnli}
     \end{subfigure}
    %  \hfill
    
    \vspace{-5pt}
    \centering
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/delta-adapter-roberta-agnews.pdf}
         \label{fig:parameter-roberta-agnews}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/delta-adapter-roberta-yahoo_answers_topics.pdf}
         \label{fig:parameter-roberta-yahoo}
     \end{subfigure}

     \vspace{-18pt}
     \begin{subfigure}[b]{0.6\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/legend.pdf}
        %  \label{fig:kshots-t5-yahoo}
     \end{subfigure}
     
    \vspace{-5pt}
    \caption{Results of tunable parameters with RoBERTa (Adapter).}
    \label{fig:parameter-roberta}
\end{figure*}


==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/fig_latex/params_roberta_soft.tex <==
\begin{figure*}[!h]
     \centering
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/delta-soft-roberta-sst2.pdf}
         \label{fig:parameter-roberta-sst2}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/delta-soft-roberta-mnli.pdf}
         \label{fig:parameter-roberta-mnli}
     \end{subfigure}
    %  \hfill
    
    \vspace{-5pt}
    \centering
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/delta-soft-roberta-agnews.pdf}
         \label{fig:parameter-roberta-agnews}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/delta-soft-roberta-yahoo_answers_topics.pdf}
         \label{fig:parameter-roberta-yahoo}
     \end{subfigure}

     \vspace{-18pt}
     \begin{subfigure}[b]{0.6\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/legend.pdf}
        %  \label{fig:kshots-t5-yahoo}
     \end{subfigure}
     
    \vspace{-5pt}
    \caption{Results of tunable parameters with RoBERTa (Soft-prompt).}
    \label{fig:parameter-roberta_soft}
\end{figure*}


==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/fig_latex/params_t5_adapter.tex <==

\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim=0 0 0 0, clip, width=\textwidth]{figures/delta-adapter-t5-sst2.pdf}
         \label{fig:adapter-t5-sst2}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim=0 0 0 0, clip,width=\textwidth]{figures/delta-adapter-t5-mnli.pdf}
         \label{fig:adapter-t5-mnli}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim=0 0 0 10, clip,width=\textwidth]{figures/delta-adapter-t5-yahoo_answers_topics.pdf}
         \label{fig:adapter-t5-yahoo}
     \end{subfigure}
     
    \vspace{-10pt}
     \begin{subfigure}[b]{0.6\textwidth}
         \centering
         \includegraphics[width=0.95\textwidth]{figures/legend.pdf}
        %  \label{fig:kshots-t5-yahoo}
     \end{subfigure}
        \vspace{-5pt}
        \caption{Results of tunable parameters with T5 (Adapter).}
        \label{fig:adapter-t5}
        % \vspace{-10pt}
\end{figure*}



==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/fig_latex/params_t5_soft.tex <==

\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim=0 0 0 0, clip, width=\textwidth]{figures/delta-soft-t5-sst2.pdf}
         \label{fig:soft-t5-sst2}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim=0 0 0 0, clip,width=\textwidth]{figures/delta-soft-t5-mnli.pdf}
         \label{fig:soft-t5-mnli}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim=0 6 0 10, clip,width=\textwidth]{figures/delta-soft-t5-yahoo_answers_topics.pdf}
         \label{fig:soft-t5-yahoo}
     \end{subfigure}
     
    \vspace{-10pt}
     \begin{subfigure}[b]{0.6\textwidth}
         \centering
         \includegraphics[width=0.95\textwidth]{figures/legend.pdf}
        %  \label{fig:kshots-t5-yahoo}
     \end{subfigure}
        \vspace{-2pt}
        \caption{Results of tunable parameters with T5 (soft prompt).}
        \label{fig:soft-t5}
\end{figure*}



==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/fig_latex/pretrain_roberta.tex <==
\begin{figure*}[!h]
     \centering
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[trim=10 20 0 0, clip, width=\textwidth]{figures/pretrain-roberta-sst2.pdf}
         \label{fig:pretrain-roberta-sst2}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[trim=10 20 0 0, clip, width=\textwidth]{figures/pretrain-roberta-mnli.pdf}
         \label{fig:pretrain-roberta-mnli}
     \end{subfigure}

     \vspace{-10pt}
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[trim=10 20 0 0, clip, width=\textwidth]{figures/pretrain-roberta-agnews.pdf}
         \label{fig:pretrain-roberta-agnews}
     \end{subfigure}
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[trim=10 20 0 0, clip, width=\textwidth]{figures/pretrain-roberta-yahoo_answers_topics.pdf}
         \label{fig:pretrain-roberta-yahoo}
     \end{subfigure}
     
    \vspace{-17pt}
     \begin{subfigure}[b]{0.64\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ figures/pretrain_legend.pdf}
     \end{subfigure}
        \vspace{-5pt}
        
        \caption{Results of the pretraining influence with RoBERTa.}
        \label{fig:pretrain_roberta}
\end{figure*}

==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/fig_latex/pretrain_t5.tex <==
\begin{figure*}[htbp]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim=10 20 0 0, clip, width=\textwidth]{figures/pretrain-t5-sst2.pdf}
         \label{fig:pretrain-t5-sst2}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim=10 20 0 0, clip, width=\textwidth]{figures/pretrain-t5-mnli.pdf}
         \label{fig:pretrain-t5-mnli}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim=10 20 0 0, clip, width=\textwidth]{figures/pretrain-t5-yahoo_answers_topics.pdf}
         \label{fig:pretrain-t5-yahoo}
     \end{subfigure}
     
    \vspace{-17pt}
     \begin{subfigure}[b]{0.64\textwidth}
         \centering
         \includegraphics[width=\textwidth]{ figures/pretrain_legend.pdf}

     \end{subfigure}
        % \vspace{pt}
        \caption{Results of the pretraining influence with T5.}
        \label{fig:pretrain}
\end{figure*}

==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/fig_latex/scale_roberta.tex <==
\begin{figure*}[h]
     \centering
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[trim=0 0 0 0, clip, width=\textwidth]{figures/scale-bert-sst2.pdf}
         \label{fig:scale-bert-sst2}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[trim=0 0 0 0, clip, width=\textwidth]{figures/scale-bert-mnli.pdf}
         \label{fig:scale-bert-mnli}
     \end{subfigure}
    %  \hfill
    
    \vspace{-5pt}
    \centering
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[trim=0 0 0 0, clip, width=\textwidth]{figures/scale-bert-agnews.pdf}
         \label{fig:scale-bert-agnews}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
     \includegraphics[trim=0 0 0 0, clip, width=\textwidth]{figures/scale-bert-yahoo_answers_topics.pdf}
     \label{fig:scale-bert-yahoo}
     \end{subfigure}

    \vspace{-15pt}
     \begin{subfigure}[b]{0.64\textwidth}
         \centering
     \includegraphics[width=\textwidth]{figures/legend_scale_roberta.pdf}
     \end{subfigure}
     
    \vspace{-5pt}
    \caption{Results of increasing PLMs scales with RoBERTa.}
    \label{fig:scale-bert}
\end{figure*}

==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/fig_latex/scale_t5.tex <==
\begin{figure*}[!h]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim=0 0 0 0, clip,width=\textwidth]{figures/scale-t5-sst2.pdf}
         \label{fig:scale-t5-sst2}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim=0 0 0 0, clip,width=\textwidth]{figures/scale-t5-mnli.pdf}
         \label{fig:scale-t5-mnli}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim=0 0 0 0, clip,width=\textwidth]{figures/scale-t5-yahoo_answers_topics.pdf}
         \label{fig:scale-t5-yahoo}
     \end{subfigure}
     
    \vspace{-12pt}
     \begin{subfigure}[b]{0.6\textwidth}
         \centering
         \includegraphics[trim=0 390 0 170, clip, width=\textwidth]{figures/legend_scale_t5.pdf}

     \end{subfigure}
        \vspace{-3pt}
        \caption{Results of increasing PLMs scales with T5.}
        % \vspace{-11pt}
        \label{fig:scale-t5}
\end{figure*}

==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/fig_latex/two-state.tex <==
\begin{figure}[]
    \vspace{-12pt}
    \centering
    \includegraphics[width=0.4\textwidth]{figures/two-states.pdf}
    \vspace{-10pt}
    \caption{The demonstration of the under-fitted and over-fitted states in the training process with RoBERTa on SST-2.}
    \label{fig:hello}
    \vspace{-15pt}
\end{figure}

==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/intro.tex <==
\section{Introduction}
% \looseness=-1
Pre-trained language models (PLMs) are successful in many downstream tasks regarding performance~\citep{DBLP:conf/iclr/WangSMHLB19}.
In high-stake applications, it's equally essential for PLMs to possess a sense of calibration~\citep{DBLP:conf/aistats/VaicenaviciusWA19}. 
% , the calibration performance should also be carefully examined
% 
% Well-calibrated models assign appropriate confidence scores that truly reflect the outcome probability of their predictions. 
% 
However, the confidence scores (a.k.a, predictive probability) of existing deep neural networks cannot serve as reliable estimates of their uncertainty~\citep{DBLP:conf/icml/GuoPSW17}, and a deep understanding of PLMs calibration is lacking. 


% especially under distribution shifts~\citep{DBLP:conf/emnlp/KongJZLZZ20}.








\input{fig_latex/two-state.tex}


In this paper, we give a systematical analysis of PLMs calibration. 
% 
We consider two questions about PLMs calibration:
(1) Do PLMs learn to become calibrated in the training process?
(2) How effective are existing calibration methods?
% 
We first introduce the metrics we adopt for calibration performance evaluation.
The most widely used calibration metric ECE (Expected Calibration Error~\cite {DBLP:conf/aaai/NaeiniCH15}) is considered. 
% 
It measures the difference between confidence and accuracy by portioning samples into various confidence zones.
%
To give a more comprehensive and practical calibration evaluation, we provide an application-driven perspective, describing two undesirable situations in practice:
(1) Correct predictions (positive) are rejected due to low confidence;
(2) Wrong predictions (negative) are accepted due to high confidence.
We propose to measure the average confidence scores on correct and wrong predictions respectively to characterize undesirable situations.
Two kinds of calibration errors are measured, denoted as CErr$_{pos}$ and CErr$_{neg}$.


% 
% \looseness=-1
For the first question, we consider the influence of six factors on PLMs' calibration performance, including dataset difficulty, available training samples, training steps, the number of tunable parameters, model scale, and pretraining.
% 
Some of them are overlooked in previous empirical studies~\citep{DBLP:conf/nips/SnoekOFLNSDRN19, DBLP:conf/cvpr/NixonDZJT19, DBLP:conf/nips/MindererDRHZHTL21}.
We motivate to conduct fine-grained control experiments to study the dynamic change in PLMs' calibration performance in training through manipulating control variables.


\looseness=-1
We empirically observe an overall consistent change in calibration performance across six factors.
% 
All six factors influence PLMs' fitness on the training distribution. 
This results in two states of PLMs considering calibration performance, namely under-fitted and over-fitted states (see Fig.\ref{fig:hello}). 
% 
In the under-fitted state, PLMs' performance and confidence increase at different speeds when more fitted on the training distribution. 
% 
In the over-fitted state, PLMs' confidence continues to increase steadily with little change in performance.
% 
\textbf{We find evidence that PLMs don't learn to become calibrated in training:
PLMs' confidence in their predictions continues to increase when more fitted on the distribution (e.g., more tunable parameters, training longer).}
This results in two miscalibration behaviors:
(1) Increasing ECE in the latter over-fitted state, and (2) Continually increasing confidence in wrong predictions, indicating that PLMs mostly don't know ``what they don't know''.
% 

We highlight our finding presents contradictory views with the two established conclusions:
(a) Larger PLMs show better calibration~\citep{srivastava2022beyond};
(b) Pretraining improves model calibration~\citep{hendrycks2019using}.
% 
We identify that the inconsistency lies in:
(1) The difficulty of evaluation datasets: the performance doesn't saturate in the considered datasets (e.g., BIG-bench~\citep{srivastava2022beyond}).
Thus, the evaluation is on the under-fitted state, leaving the miscalibration behavior in the over-fitted state unobserved;
(2) Evaluation metrics: previous work doesn't measure the confidence in wrong predictions, overlooking the fact that models are becoming more confident in wrong predictions when scaling larger and employing pretraining.

% We elaborate the arguments later in Sec.~\ref{sec:empirical_study}. 


% (1) PLMs' confidence continues to increase when more fitted on the distribution , while the performance score may converge earlier. This may result in increasing ECE in the latter stage; 
% (2) Worse, the confidence in wrong predictions also holds the consistent increasing trend in the fitting process. 
% This is undesirable in practice since wrong predictions may be accepted due to high confidence, and indicates that PLMs mostly don't know ``what they don't know'.
% conduct a fine-grained analysis to quantify the influence of six factors on PLMs calibration. 
% We draw a general conclusion:
% \textit{The calibration performance is highly determined by PLMs' fitness on the training distribution.} 
% We observe two stages, , in the fitting process that PLMs' calibration performance shows different trends. 
% The trends hold consistently among the explored six factors that dynamically influence PLMs' fitness.

% \looseness=-1




% which is dynamically influenced by identified six dimensions.}






% To further understand PLMs calibration, we present a fine-grained empirical study, exploring the influence of six dimensions on calibration performance. 
% Based on the analysis, we move towards practicality, and investigate existing calibration methods, partitioned into unlearnable and learnable groups, in both in-distribution and out-of-distribution settings. 

% present a comprehensive study, including a fine-grained analysis spanning six dimensions. 

% four identified factors' influence, reexamination of established conclusions, and calibration methods in both in-distribution and out-of-distribution settings.

% \looseness=-1





% However, ECE alone cannot capture instance-level calibration error, and has cancellation effects~\citep{si2022revisiting}. 
% We provide an application-driven perspective for complementary evaluation, describing two undesirable situations in practice.  
% Two metrics mentioned in~\cite{si2022revisiting} are adopted: 
% (1) CErr$_{pos}$, characterizing the error of giving low confidence scores on correct predictions;
% (2) CErr$_{neg}$, characterizing the error of giving high confidence scores on wrong predictions. 
% 





% We elaborate the last two metrics in Sec.~\ref{sec:exp_setting}.
% We adopt two metrics, CErr$_{pos}$ and CErr$_{neg}$, to characterize two undesirable situations in practice: (1) Reject correct predictions due to low confidence; (2) Accept wrong predictions due to high confidence. 
% In our study, we consider three calibration metrics: 
% (1) ECE~\citep{}, the most widely adopted metric; (2) 


% We consider six dimensions that may influence PLMs calibration, some of them are overlooked in previous empirical studies.
% First, we identify four factors that have significant influences on model calibration, which are often overlooked in previous empirical studies~\citep{}. 
% The six dimensions are dataset difficulty, available training sample, training step, number of tunable parameter, model scale, and pretraining. 
% We conduct a fine-grained analysis, aiming to quantify their influence on PLMs calibration. 
% We find a consistent trend and conclusion across six dimensions: 

% This dynamic process can be overall summarized as:
% (1) PLMs' performance scores and confidence increase at different speeds;


% For example, increasing the PLMs scale on hard datasets (e.g., BIG-bench) continues to bring up performance. \yang{add here}
% However, scaling larger only bring






% There is no significant difference in PLMs' confidence between correct and wrong predictions. 





% and summarize the main findings of our results as follows: 

% \begin{itemize} [topsep=1pt, partopsep=1pt, leftmargin=12pt, itemsep=0pt]
%     \item We take a close look at some critical points. 
%     We find that the increase or decrease in ECE can be estimated according to different increasing rates of model performance and confidence. 
%     Typically, miscalibration is due to the mismatch between two trends, where a larger increasing rate in performance reduces ECE and vice versa.
    
%     % \item There exists a strong and consistent correlation between models' average confidence in all predictions, correct predictions, and wrong predictions. 
%     \item PLMs' average confidence scores on all predictions, correct predictions, and wrong predictions continually increase as models become more proficient on the task.  
%     % As models become more proficient on the task, their predictions, whether correct or wrong, will continually become more confident. 
%     Namely, there is no significant difference in model confidence between correct and wrong predictions. 
%     This is undesirable in practice since we may accept wrong predictions due to their high confidence, and indicates that models don't actually learn to become more calibrated in the training process.    
    
%     \item More training steps and tunable parameters continue to increase PLMs' confidence in their predictions, even though the accuracy may have reached a plateau value.  
%     After model performance converges, training longer or increasing model capacity potentially brings a negative impact on PLMs calibration. 
%     Besides, it reveals that previous conclusions drawn from empirical studies should be carefully examined since ECE is sensitive to the training paradigm, which may be different between model architectures and calibration methods, thus resulting in unfair comparisons. 
    
% \end{itemize}



% Given the analysis of model capacity on calibration, we consider two conclusions in previous works:
% (1) Larger pre-trained language models show better calibration~\citep{srivastava2022beyond}; 
% (2) Pretraining improves model calibration~\citep{hendrycks2019using}.
% The main findings are: 
% \begin{itemize} [topsep=1pt, partopsep=1pt, leftmargin=12pt, itemsep=0pt]
%     \item Increasing the model scale cannot guarantee better calibration score (e.g., ECE). 
%     Once the scaling doesn't bring substantial improvement to the performance, ECE will increase due to the continual increase in model confidence throughout the scaling process.  
%     Worse, models continue to become more confident on wrong predictions in the scaling process, indicating that larger models do not actually learn to be calibrated on their predictions.
%     % Thus, it's a dataset-specific choice to incorporate the scaling strategy to improve model calibration. 
%     \item While pretraining consistently increases models' confidence in their predictions across different datasets, it doesn't consistently achieve better ECE compared to non-pretrained models (e.g., bag-of-word, LSTM). 
%     % Still, it's a dataset-specific choice, and the reliable conclusion is that pretraining improves model capacity, which will generally increase models' confidence. 
%     Thus, it's unsafe to conclude that pretraining improves model calibration.
    
% \end{itemize}














% conduct a comprehensive empirical study in model calibration. 
% Different from previous works that stick to the common evaluation setting and metrics (e.g., ECE)~\citep{DBLP:conf/nips/SnoekOFLNSDRN19, DBLP:conf/cvpr/NixonDZJT19, DBLP:conf/nips/MindererDRHZHTL21}, 
% we in addition (1) conduct a fine-grained analysis of multiple factors' influence on model calibration, including the number of available samples, the training steps, the number of tunable parameters, calibration methods, and the out-of-distribution evaluation datasets, and
% (2) introduce application-driven metrics to measure model calibration from a new perspective. 



% Our metrics measure the instance-level calibration error considering undesirable cases in practice.
% We draw inspiration from \cite{si2022revisiting}, and our intuition is that desirable calibrated models should give high confidence in their correct predictions while assigning low confidence to wrong ones.
 


% Based on the fine-grained understanding of PLMs calibration, we study the influence of existing calibration methods in both in-distribution and out-of-distribution (OOD) settings to situate the PLMs calibration problem in practice. 
% Finally, we study different calibration methods in both  
% \looseness=-1
Thus, we find that the main issue of PLMs calibration lies in their overconfidence in wrong predictions, which cannot be trivially solved by increasing the model scale. 
So we consider the effectiveness of existing calibration methods in mitigating the overconfidence issue. 
% 
% influence of distribution shifts and existing calibration methods on PLMs' calibration performance.
We partition existing calibration methods into unlearnable and learnable groups.
% 
Unlearnable methods heuristically manipulate the original confidence in predictions (e.g., label smoothing).
% 
Learnable methods directly collect data and train models to give reasonable confidence scores in their predictions.  
% 
Namely, an extra calibration task is introduced, which aims to extract features from samples and models' preceding performance to predict whether models' predictions are correct or not.
% For a comprehensive study of OOD shifts, we consider three different settings, namely standard distribution shifts, hard-to-easy shifts, and receiving task-irrelevant inputs (e.g., plain text, random tokens). 




\looseness=-1
\textbf{In our experiments, we identify the superiority of learnable methods compared to unlearnable ones, considering both in-distribution (ID) and out-of-distribution (OOD) settings.} 
This is characterized by a sharp decrease in their confidence in wrong predictions when using learnable methods, indicating that they significantly mitigate the overconfidence issue. 
% 
Moreover, learnable methods can maintain a reasonable increase in CErr$_{pos}$, holding consistent correlations between the drop in confidence and performance under distribution shifts.
% 
This shows the difference from unlearnable methods, which  take effect by roughly imposing confidence regularization on models' predictions (e.g., label smoothing), resulting in almost the same amount of increase in CErr$_{pos}$ with the decrease in CErr$_{neg}$. 


% \textbf{In our experiments, we identify that learnable calibration methods significantly mitigate the overconfidence issue, characterized by a sharp decrease in their confidence in wrong predictions, considering both in-distribution (ID) and out-of-distribution (OOD) settings.}
% 

% 
% This shows the advantage of learnable methods compared to unlearnable ones (e.g., label smoothing),
% which
% 
% 
% Besides, to further improve or maintain PLMs calibration without sacrificing the original task performance, we propose three simple extended calibration methods based on the adapted learnable ones~\citep{lin2022teaching, kadavath2022language}.
% Experimental results show the superiority of our methods.




% the average confidence drop is highly relevant with the performance drop under distribution shifts. Thus, the relatively higher CErr$_{pos}$ on OOD samples may be reasonable.

\looseness=-1
To further understand learnable calibration methods, we consider the influence of more data and larger model scales for the calibration task, the adopted model for the calibration task, and the data distribution, on PLMs' calibration performance. 
% 
We highlight three findings:
(1) More data and larger model scales for the calibration task both play significant positive roles in PLMs' calibration performance;
% 
(2) PLMs can be trained to give their uncertainty. This finding is consistent with the concurrent work~\citep{lin2022teaching}.
% proposes a learnable method and draws the conclusion that language models can be trained to give uncertainty estimation of their predictions by words.
Further, we provide an extension to this conclusion. 
We find that using an extrinsic predictive model can achieve comparable results, given the same calibration training data. 
% 
Thus, we identify that the success of this paradigm essentially lies in the learnable attribute of the calibration task, instead of the PLMs' self-checking process;
% 
(3) PLMs' calibration performance under distribution shifts depends on the evaluation datasets chosen. 
Previous work shows that PLMs exhibit degraded calibration performance under distribution shifts~\citep{DBLP:conf/emnlp/DesaiD20}. 
% 
We find that this conclusion is reversed when the ID datasets are harder and PLMs achieve better performance on OOD datasets.
% 
The concrete arguments and explanations are detailed in Appendix \ref{sec:further_dis}.




% To further exploit and understand learnable calibration methods, we investigate the influence of more data and larger model scale for the calibration task on calibration performance.
% the dataset size for the calibration task and model scale on the calibration performance.
% 
% We find that they both play significant positive roles in PLMs' calibration performance.
% But the overall trends are different between two factors and across evaluation settings. 
% We detail the findings in Sec.~\ref{sec:emergent}.
% 
% Finally, we highlight that our analysis results provide extensions to two existing findings:








% we consider the conclusion in~ that 
% 


% Specifically, increasing the dataset size improves PLMs calibration before a critical point, after which the influence is negligible. 
% Scaling larger shows consistent improvement on PLMs calibration considering all evaluation metrics on ID samples. 
% For distribution shifts, we don't observe a consistent trend. 




% Our main findings are:
% (1) Increasing the dataset size has significant influence on PLMs calibration before a critical point, after which the influence is negligible. 
% PLMs show better calibration performance in this process since their confidence in wrong predictions drop significantly on ID samples;
% (2) Scaling larger shows 



% But we also find a trade-off since learnable methods also decrease the confidence in correct predictions, especially under distribution shifts. Here we provide two observations indicating that learnable methods essentially teach models to have clear confidence estimations:
% (1) The increase in CErr$_{pos}$ is significantly lower than the decrease in CErr$_{neg}$.
% For reference, the most effective unlearnable methods (e.g., temperature scaling and label smoothing) take effect by , resulting in ;
% % thus don't actually teach models to have clear confidence estimations of their predictions. 
% (2) Learnable methods give obviously lower confidence in OOD samples, and the average confidence drop is highly relevant with the performance drop under distribution shifts. Thus, the relatively higher CErr$_{pos}$ on OOD samples may be reasonable.





    

% This is reasonable when evaluated on OOD samples that models may be unfamiliar with. 
    
    
    

 
 
%  For unlearnable methods, while incorporating model ensemble and data augmentation techniques don't show substantial differences with the vanilla fine-tuning, temperature scaling and label smoothing reduce ECE and remain strong baseline methods.  
    % However, these two methods 



% There also exists a trade-off when adopting learnable methods since the confidence in correct predictions also decreases, especially under distribution shifts.
    % There also exists a trade-off between CErr$_{pos}$ and CErr$_{neg}$ when adopting learnable methods, especially under distribution shifts.
    % PLMs with learnable methods tend to obtain higher CErr$_{pos}$, meaning that they are less confident on their correct predictions.
   
    
    
    
% We summarize the main findings as follows: 
% \begin{itemize} [topsep=1pt, partopsep=1pt, leftmargin=12pt, itemsep=0pt]
    
%     \item   
    % Considering all methods, PLMs are significantly less calibrated under standard distribution shifts.
    % It's due to the severe mismatch between performance and confidence.
    % Interestingly, we observe a reverse trend when evaluated under hard-to-easy shifts.
    % We identify that the  influence of distribution shifts on PLMs calibration is dependent on the evaluation datasets chosen, and the conclusion that PLMs are less calibrated under distribution shifts is one-sided. 
    % Overall, we find PLMs mostly don’t know “what they don’t know” since they consistently assign high confidence to wrong predictions.
    
    
   
    
    % significantly reducing models' confidences on their predictions.
    % This is undesirable for correct predictions since they may be falsely rejected due to relatively low confidence. 
    % Thus, we argue that although roughly reducing models' confidence may be a solution to achieving low ECE, it doesn't actually help models to have a clear estimation of their predictions. 
    % \item PLMs show unreasonably high predicted confidence in task-irrelevant inputs, especially when trained on relatively simple in-distribution datasets (e.g., SST-2). 
    % Thus, we conclude that the difficulty of the training dataset has a substantial influence on model calibration. 
    % The results further support our identified influence factors that impact PLMs calibration. 
    
  
    
    

% We hypothesize that there also exists a calibration problem in the calibration task. 
% Thus, it's important to find an appropriate model scale for the calibration task. 





% We then propose a simple method to train calibrated models. 
% \begin{figure*}
%     \centering
%     \includegraphics[trim=20 80 120 50, clip ,width=\textwidth]{figures/hello_fig.pdf}
%     \caption{Pipeline}
%     \label{fig:pipeline}
% \end{figure*}





 









==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/reexam.tex <==
% \section{Reexamining established conclusions}

% \label{sec:reexam}
% We reexamine two established conclusions in previous works: (1) Larger PLMs are more calibrated~\citep{srivastava2022beyond};
% % Specifically, 
% (2) Pretraining improves model calibration~\citep{hendrycks2019using}.


==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/rel.tex <==

\section{Background}
\label{sec:background}
\paragraph{Calibration measure.}
% Given unlimited data, proper scoring rules~\citep{gneiting2007probabilistic} like cross-entropy loss ensure the training algorithm to yield well-calibrated models. 
% However, in practice, miscalibration happens due to overfitting on available training samples.
\looseness=-1
We can visualize model calibration through reliability diagram~\citep{degroot1983comparison}.
% 
Based on the diagram, we can measure the ECE~\citep{DBLP:conf/aaai/NaeiniCH15} by partitioning samples into different confidence zones.
The central idea is to measure the absolute difference between models' predictive confidence and accuracy.
Although alternative theoretic-motivated metrics have been proposed~\citep{DBLP:conf/aistats/VaicenaviciusWA19, DBLP:conf/iclr/GuptaRAMS021}, we still employ ECE in our experiments due to its simplicity and popularity.
% Besides, we also provide an application-driven perspective to look into model calibration. 


\paragraph{Benchmark \& Analysis.}
Given appropriate evaluation metrics, large-scale benchmarks have been conducted to analyze model calibration under different settings, spanning model architectures~\citep{DBLP:conf/icml/GuoPSW17, DBLP:conf/nips/MindererDRHZHTL21}, model scales~\citep{DBLP:conf/emnlp/DanR21}, modalities~\citep{DBLP:conf/emnlp/DesaiD20,DBLP:conf/nips/MindererDRHZHTL21, kadavath2022language}, calibration methods~\citep{DBLP:conf/icml/GuoPSW17, DBLP:conf/emnlp/DesaiD20}, and distribution shifts~\citep{DBLP:conf/cvpr/NixonDZJT19, DBLP:conf/emnlp/KongJZLZZ20}. 
% 
Our work is closely related to~\citet{xiao2022uncertainty} that quantifies the uncertainty of PLMs. 
% 
However, previous benchmarks follow the fixed training and evaluation paradigms.
% 
In this paper, we instead conduct a fine-grained and more comprehensive empirical evaluation to take a close look into PLMs calibration from multiple dimensions that have often been overlooked. 
% 
Also, we consider and conduct a detailed analysis of the recently proposed learnable calibration methods~\citep{lin2022teaching, kadavath2022language}.
% 




% We control different factors in our study, including training dynamics, number of available samples and tunable parameters, calibration methods, and distribution shifts.
% We draw new conclusions from experiments based on our new established perspective. 






\paragraph{Method.}
Calibration is essential for out-of-distribution detection~\citep{hendrycks2019scaling}, selective prediction~\citep{varshney2022investigating}, robustness~\citep{kumar2022calibrated}, and pseudo-labeling~\citep{rizve2021defense}. 
Existing calibration methods can be partitioned into unlearnable and learnable groups. 
For unlearnable methods, there are mainly four categories.
Post-hoc calibration intends to readjust the output logits referring to the performance on a held-out validation set~\citep{platt1999probabilistic, DBLP:conf/icml/GuoPSW17}. 
Regularization methods aim to prevent models from being over-confident on predictions~\citep{DBLP:conf/cvpr/SzegedyVISW16, DBLP:conf/iclr/PereyraTCKH17}. 
Data augmentation~\citep{DBLP:conf/iclr/HendrycksMCZGL20, DBLP:conf/nips/WangXKYAW21} and model ensemble~\citep{DBLP:conf/icml/GalG16, DBLP:conf/nips/Lakshminarayanan17} have also been empirically proven to improve model calibration.
For learnable methods, the typical way is to first collect data for the calibration task, and then train a model to predict whether the given answer is correct. 
The model can be a multi-layer perceptron, and the features can be hand-engineered~\citep{DBLP:conf/acl/YeD22, DBLP:conf/acl/ZhangGC21, si2022revisiting} or the last hidden states of PLMs~\citep{kadavath2022language}. 
PLMs can also be directly trained to output their uncertainty by words~\citep{lin2022teaching}.

% In NLP, there is a growing trend in examining the calibration of large pretrained language models~\citep{DBLP:conf/iclr/HendrycksBBZMSS21, DBLP:journals/corr/abs-2205-14334, kadavath2022language} due to their strong capacity~\citep{brown2020language, wei2021finetuned}.
% % In this paper, we also focus on the NLP filed due to the practical few-shot learning~\citep{DBLP:conf/eacl/SchickS21, DBLP:conf/acl/GaoFC20}, parameter-efficient learning~\citep{DBLP:conf/icml/HoulsbyGJMLGAG19, DBLP:journals/corr/abs-2106-09685, DBLP:conf/acl/ZakenGR22}, and in-context learning for large language models~\citep{brown2020language, zhang2022opt}. 













==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/tab/calibration_template.tex <==

\begin{table*}[t!]
\renewcommand{\arraystretch}{1.3}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}l|l|l|l@{}}
\toprule
Task                                                                          & Dataset        & Template                                                                                                                                                                                                                                     & Verbalizer        \\ \midrule
                                                                              & SST-2          & \begin{tabular}[c]{@{}l@{}}Sentence: \{"placeholder": "text\_a"\} The predicted sentiment is \{"placeholder": "text\_b"\} . \\ Is the prediction True or False ? It's \{"mask"\} .\end{tabular}                                              &                   \\ \cmidrule(lr){2-3}
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}~\\Sentiment\\ Analysis\end{tabular}} & Amazon         & \begin{tabular}[c]{@{}l@{}}Sentence: \{"placeholder": "text\_a"\} The predicted sentiment is \{"placeholder": "text\_b"\} . \\ Is the prediction True or False ? It's \{"mask"\} .\end{tabular}                                              &                   \\ \cmidrule(lr){2-3}
                                                                              & SST-5          & \begin{tabular}[c]{@{}l@{}}Sentence: \{"placeholder": "text\_a"\} The predicted sentiment is \{"placeholder": "text\_b"\} . \\ Is the prediction True or False ? It's \{"mask"\} .\end{tabular}                                              &                   \\ \cmidrule(lr){2-3}
                                                                              & SemEval        & \begin{tabular}[c]{@{}l@{}}Sentence: \{"placeholder": "text\_a"\} The predicted sentiment is \{"placeholder": "text\_b"\} . \\ Is the prediction True or False ? It's \{"mask"\} .\end{tabular}                                              &                   \\ \cmidrule(r){1-3}
                                                                              & MNLI           & \begin{tabular}[c]{@{}l@{}}Given the two sentences: \{"placeholder": "text\_a"\} \\ The predicted relationship between the two sentences is \{"placeholder": "text\_b"\} \\ Is the prediction True or False ? It's \{"mask"\} .\end{tabular} &                   \\ \cmidrule(lr){2-3}
\begin{tabular}[c]{@{}l@{}}Natural\\ Language \\ Inference\end{tabular}       & HANS           & \begin{tabular}[c]{@{}l@{}}Given the two sentences: \{"placeholder": "text\_a"\} \\ The predicted relationship between the two sentences is \{"placeholder": "text\_b"\} \\ Is the prediction True or False ? It's \{"mask"\} .\end{tabular} & {[}False, True{]} \\ \cmidrule(lr){2-3}
                                                                              & ANLI           & \begin{tabular}[c]{@{}l@{}}Given the two sentences: \{"placeholder": "text\_a"\} \\ The predicted relationship between the two sentences is \{"placeholder": "text\_b"\} \\ Is the prediction True or False ? It's \{"mask"\} .\end{tabular} &                   \\ \cmidrule(r){1-3}
\begin{tabular}[c]{@{}l@{}}Topic\\ Classification\end{tabular}                & Yahoo          & \begin{tabular}[c]{@{}l@{}}Sentence: \{"placeholder": "text\_a"\} The predicted topic is \{"placeholder": "text\_b"\} \\ Is the prediction True or False ? It's \{"mask"\} .\end{tabular}                                                    &                   \\ \cmidrule(r){1-3}
                                                                              & Civil          & \begin{tabular}[c]{@{}l@{}}Sentence: \{"placeholder": "text\_a"\} The predicted toxicity is \{"placeholder": "text\_b"\} . \\ Is the prediction True or False ? It's \{"mask"\} .\end{tabular}                                               &                   \\ \cmidrule(lr){2-3}
\begin{tabular}[c]{@{}l@{}}Toxic\\ Detection\end{tabular}                     & Hate Speech    & \begin{tabular}[c]{@{}l@{}}Sentence: \{"placeholder": "text\_a"\} The predicted toxicity is \{"placeholder": "text\_b"\} . \\ Is the prediction True or False ? It's \{"mask"\} .\end{tabular}                                               &                   \\ \cmidrule(lr){2-3}
                                                                              & Implicite Hate & \begin{tabular}[c]{@{}l@{}}Sentence: \{"placeholder": "text\_a"\} The predicted toxicity is \{"placeholder": "text\_b"\} . \\ Is the prediction True or False ? It's \{"mask"\} .\end{tabular}                                               &                   \\ \bottomrule
\end{tabular}

}

\caption{The manual templates and verbalizers of the calibration task for each dataset.}
\label{tab:calibration_template}
\end{table*}

==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/tab/datasets.tex <==
\begin{table*}[t]
\centering
% \vspace{-20pt}

\resizebox{0.75\textwidth}{!}{
\begin{tabular}{@{}l|l|ccccc@{}}
\toprule
Task                                                                                    & Dataset       & \# Classes & Avg.Len     & Train  & Dev   & Test  \\ \midrule
                                                                                        & SST-2         & 2          & 19.23       & 6920   & 1821  & 872   \\
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Sentiment\\ Analysis\end{tabular}}           & Amazon        & 3          & 77.86       & 24000  & 78741 & 91606 \\
                                                                                        & SST-5         & 3          & 18.75       & -      & -     & 1067  \\
                                                                                        & SemEval       & 3          & 19.61       & -      & -     & 6000  \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Natural\\ Language\\ Inference\end{tabular}} & MNLI          & 3          & 19.36/10.06 & 373067 & 19635 & 9815  \\
                                                                                        & HANS          & 2          & 9.15/5.61   & -      & -     & 30000 \\
                                                                                        & ANLI          & 3          & 54.40/10.34 & -      & -     & 3200  \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Topic\\ Classification\end{tabular}}         & Yahoo         & 10         & 96.98       & 126000 & 14000 & 60000 \\
                                                                                        & AG            & 4          & 38.5        & 10000  & -     & 7600  \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Toxic\\ Detection\end{tabular}}              & Civil         & 2          & 52.86       & 48000 & 12000 & 97320 \\
                                                                                        & Hate Speech   & 2          & 21.55       & -      & -     & 478   \\
                                                                                        & Implicit Hate & 2          & 17.34       & -      & -     & 21479 \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Plain\\ Text\end{tabular}}                   & Book Corpus   & -          & 13.39       & -      & -     & 10000 \\
                                                                                        & Random Words  & -          & 20.28       & -      & -     & 1000  \\ \bottomrule
\end{tabular}
}
\caption{Dataset Statistics.}
% \vspace{-30pt}
\label{tab:statistics}
\end{table*}

==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/tab/emergent.tex <==
\begin{table*}[]
\caption{Results on the emergent calibration of T5 with increasing dataset sizes.}

\resizebox{\textwidth}{!}{

\begin{tabular}{@{}l|l|ccccc|ccccc|ccccc@{}}
\toprule
Dataset Size              & Dataset     & \multicolumn{5}{c|}{Amazon}                                               & \multicolumn{5}{c|}{SST-5}                                                & \multicolumn{5}{c}{SemEval}                                                        \\ \midrule
\multirow{6}{*}{Small}    & Method      & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf           & ECE            & CErr$_{pos}$   & CErr$_{neg}$   \\ \cmidrule(l){2-17} 
                          & E-MLP       & 89.19          & 90.27 & 9.13           & \textbf{9.13}  & 85.30          & \textbf{67.67} & 84.41 & \textbf{18.54} & 14.93          & 83.01          & 55.02          & 82.55          & \textbf{27.85} & \textbf{16.43} & 81.30          \\
                          & E-T5        & 89.19          & 78.74 & \textbf{8.81}  & 11.41          & 31.68          & \textbf{67.67} & 79.97 & 25.61          & 14.36          & 69.96          & 55.02          & 56.08          & 31.55          & 40.78          & 52.11          \\
                          & I-Vanilla   & 88.87          & 78.15 & 9.18           & 12.02          & 30.66          & 65.98          & 75.80 & 26.17          & 18.35          & 65.82          & 55.85          & 54.67          & 31.24          & 41.76          & 50.02          \\
                          & I-Iterative & 90.04          & 80.20 & 10.23          & 10.70          & 45.30          & 66.54          & 86.12 & 24.57          & \textbf{10.60} & 80.07          & \textbf{56.40} & 62.44          & 27.98          & 35.61          & 59.53          \\
                          & I-Multitask & \textbf{90.23} & 78.22 & 8.98           & 10.02          & \textbf{21.84} & 67.10          & 56.76 & 26.16          & 31.65          & \textbf{38.75} & 55.87          & 45.78          & 37.04          & 49.90          & \textbf{39.48} \\ \midrule
\multirow{6}{*}{Middle}   & Method      & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf           & ECE            & CErr$_{pos}$   & CErr$_{neg}$   \\ \cmidrule(l){2-17} 
                          & E-MLP       & 89.19          & 89.82 & \textbf{6.92}  & \textbf{8.83}  & 78.70          & 67.67          & 81.30 & \textbf{15.72} & \textbf{17.30} & 78.37          & 55.02          & 79.01          & \textbf{24.05} & \textbf{19.45} & 77.13          \\
                          & E-T5        & 89.19          & 68.57 & 10.94          & 13.77          & 2.56           & 67.67          & 28.37 & 30.89          & 54.59          & 9.20           & 55.02          & 15.76          & 43.77          & 77.17          & 6.56           \\
                          & I-Vanilla   & 87.31          & 67.79 & 12.94          & 15.87          & \textbf{2.50}  & \textbf{65.51} & 24.90 & 33.68          & 59.76          & 6.96           & 51.50          & 15.26          & 47.71          & 78.96          & 6.62           \\
                          & I-Iterative & \textbf{90.65} & 69.70 & 9.82           & 12.20          & 3.28           & 67.10          & 20.65 & 32.25          & 64.03          & \textbf{5.01}  & \textbf{55.33} & \textbf{9.79}  & 44.08          & 85.07          & \textbf{4.25}  \\
                          & I-Multitask & 90.21          & 69.35 & 9.84           & 12.48          & 2.81           & 67.48          & 28.73 & 31.28          & 54.11          & 7.49           & \textbf{54.93} & 17.34          & 44.74          & 75.11          & 6.89           \\ \midrule
\multirow{6}{*}{Large}    & Method      & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf           & ECE            & CErr$_{pos}$   & CErr$_{neg}$   \\ \cmidrule(l){2-17} 
                          & E-MLP       & 89.19          & 89.95 & \textbf{5.34}  & \textbf{8.38}  & 76.06          & 67.76          & 79.66 & \textbf{14.11} & \textbf{18.61} & 76.03          & 55.03          & 78.22          & \textbf{23.13} & \textbf{19.94} & 75.96          \\
                          & E-T5        & 89.19          & 69.06 & 11.05          & 13.81          & \textbf{2.76}  & 67.76          & 26.04 & 30.98          & 57.08          & 6.54           & 55.03          & 12.85          & 44.42          & 80.71          & 4.99           \\
                          & I-Vanilla   & 88.52          & 69.48 & 11.66          & 14.40          & 3.05           & \textbf{68.13} & 24.56 & 30.75          & 58.11          & \textbf{5.65}  & 47.73          & 12.05          & 52.10          & 83.63          & 4.98           \\
                          & I-Iterative & \textbf{91.09} & 69.27 & 9.40           & 12.04          & 3.60           & 66.82          & 25.01 & 31.65          & 59.16          & 7.38           & 55.03          & 9.28           & 44.90          & 85.61          & \textbf{3.71}  \\
                          & I-Multitask & 90.21          & 69.01 & 10.18          & 13.10          & 3.23           & 67.20          & 28.78 & 30.99          & 54.73          & 8.46           & \textbf{55.90} & 14.81          & 43.28          & 77.88          & 5.72           \\ \midrule
Model Scale               & Dataset     & \multicolumn{5}{c|}{Amazon}                                               & \multicolumn{5}{c|}{SST-5}                                                & \multicolumn{5}{c}{SemEval}                                                        \\ \midrule
\multirow{6}{*}{T5-small} & Method      & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf           & ECE            & CErr$_{pos}$   & CErr$_{neg}$   \\ \cmidrule(l){2-17} 
                          & E-MLP       & 85.51          & 85.87 & \textbf{10.87} & \textbf{13.00} & 79.17          & 60.82          & 77.84 & \textbf{19.95} & \textbf{21.30} & 76.51          & 47.13          & 76.62          & \textbf{30.41} & \textbf{21.86} & 75.27          \\
                          & E-T5        & 85.51          & 63.09 & 15.18          & 19.73          & \textbf{4.31}  & 60.82          & 20.19 & 37.67          & 68.27          & 6.40           & 47.13          & 24.11          & 49.85          & 72.19          & 16.02          \\
                          & I-Vanilla   & 74.41          & 58.28 & 25.89          & 31.18          & 4.64           & 57.08          & 19.47 & 41.64          & 71.05          & 6.41           & 47.85          & 24.84          & 49.14          & 71.30          & 16.68          \\
                          & I-Iterative & \textbf{86.64} & 64.97 & 14.55          & 19.06          & 5.64           & \textbf{60.92} & 17.68 & 37.90          & 71.69          & 5.35           & \textbf{49.43} & 21.98          & 46.06          & 74.32          & 15.22          \\
                          & I-Multitask & 84.87          & 59.20 & 16.78          & 22.53          & 4.70           & 57.92          & 11.50 & 41.83          & 81.10          & \textbf{3.42}  & 48.65          & \textbf{15.41} & 49.94          & 80.43          & \textbf{8.41}  \\ \midrule
\multirow{6}{*}{T5-base}  & Method      & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf           & ECE            & CErr$_{pos}$   & CErr$_{neg}$   \\ \cmidrule(l){2-17} 
                          & E-MLP       & 89.19          & 89.82 & \textbf{6.92}  & \textbf{8.83}  & 78.70          & 67.67          & 81.30 & \textbf{15.72} & \textbf{17.30} & 78.37          & 55.02          & 79.01          & \textbf{24.05} & \textbf{19.45} & 77.13          \\
                          & E-T5        & 89.19          & 68.57 & 10.94          & 13.77          & 2.56           & 67.67          & 28.37 & 30.89          & 54.59          & 9.20           & 55.02          & 15.76          & 43.77          & 77.17          & 6.56           \\
                          & I-Vanilla   & 87.31          & 67.79 & 12.94          & 15.87          & \textbf{2.50}  & \textbf{65.51} & 24.90 & 33.68          & 59.76          & 6.96           & 51.50          & 15.26          & 47.71          & 78.96          & 6.62           \\
                          & I-Iterative & \textbf{90.65} & 69.70 & 9.82           & 12.20          & 3.28           & 67.10          & 20.65 & 32.25          & 64.03          & \textbf{5.01}  & \textbf{55.33} & \textbf{9.79}  & 44.08          & 85.07          & \textbf{4.25}  \\
                          & I-Multitask & 90.21          & 69.35 & 9.84           & 12.48          & 2.81           & 67.48          & 28.73 & 31.28          & 54.11          & 7.49           & \textbf{54.93} & 17.34          & 44.74          & 75.11          & 6.89           \\ \midrule
\multirow{6}{*}{T5-large} & Method      & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf           & ECE            & CErr$_{pos}$   & CErr$_{neg}$   \\ \cmidrule(l){2-17} 
                          & E-MLP       & 91.14          & 91.65 & \textbf{4.89}  & \textbf{7.04}  & 78.18          & 69.17          & 83.16 & \textbf{17.31} & \textbf{15.40} & 79.94          & 54.35          & 77.30          & \textbf{22.95} & \textbf{21.60} & 75.99          \\
                          & E-T5        & 91.14          & 70.61 & 8.84           & 11.16          & 2.20           & 69.17          & 25.63 & 29.27          & 56.81          & 6.87           & 54.35          & 22.29          & 43.22          & 70.85          & 10.87          \\
                          & I-Vanilla   & 89.51          & 70.08 & 10.56          & 13.02          & \textbf{2.05}  & 68.98          & 24.66 & 29.46          & 57.82          & \textbf{6.30}  & 51.72          & 21.36          & 45.84          & 72.78          & \textbf{10.65} \\
                          & I-Iterative & \textbf{92.72} & 73.49 & 7.28           & 9.11           & 2.89           & \textbf{70.67} & 25.57 & 27.48          & 56.57          & 7.67           & \textbf{59.00} & 26.49          & 37.00          & 65.23          & 14.23          \\
                          & I-Multitask & 91.83          & 70.99 & 8.58           & 10.61          & 3.01           & 70.10          & 26.95 & 28.78          & 55.11          & 8.16           & 57.13          & 21.52          & 40.13          & 70.71          & 10.81          \\ \bottomrule
\end{tabular}

}


\label{tab:emergent_dev_size}
\end{table*}

==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/tab/emergent_devset_size.tex <==
\begin{table*}[t]


\resizebox{\textwidth}{!}{

\begin{tabular}{@{}l|l|ccccc|ccccc|ccccc@{}}
\toprule
Dataset Size            & Dataset   & \multicolumn{5}{c|}{Amazon}                                             & \multicolumn{5}{c|}{SST-5}                                                & \multicolumn{5}{c}{SemEval}                                                        \\ \midrule
\multirow{6}{*}{Small}  & Method    & Acc            & Conf  & ECE           & CErr$_{pos}$  & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf           & ECE            & CErr$_{pos}$   & CErr$_{neg}$   \\ \cmidrule(l){2-17} 
                        & E-MLP     & 91.00          & 90.41 & \textbf{1.71} & \textbf{9.59} & 90.39          & \textbf{69.73} & 87.81 & 18.08          & \textbf{12.16} & 87.73          & \textbf{55.03} & 86.86          & 31.83          & \textbf{13.11} & 86.83          \\
                        & E-T5 \ours     & 91.00          & 68.92 & 22.08         & 28.16         & 39.44          & \textbf{69.73} & 55.95 & 15.12          & 41.71          & 50.58          & \textbf{55.03} & 50.99          & \textbf{8.54}  & 43.17          & 43.84          \\
                        & I-Vanilla & 89.06          & 68.45 & 20.61         & 28.01         & 39.62          & 63.92          & 56.49 & \textbf{10.66} & 39.82          & 49.96          & 51.48          & 49.47          & 9.12           & 44.10          & 42.64          \\
                        & I-Iter \ours    & 90.58          & 68.96 & 21.62         & 28.08         & 40.47          & 69.63          & 56.69 & 12.95          & 41.27          & 52.00          & 53.72          & 53.89          & 10.24          & 43.31          & 50.64          \\
                        & I-Simul \ours   & \textbf{91.37} & 80.44 & 15.44         & 15.05         & \textbf{32.78} & 71.13          & 66.28 & 26.97          & 25.58          & \textbf{46.23} & 54.08          & \textbf{37.51} & 34.94          & 53.82          & \textbf{27.30} \\ \midrule
\multirow{6}{*}{Middle} & Method    & Acc            & Conf  & ECE           & CErr$_{pos}$  & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf           & ECE            & CErr$_{pos}$   & CErr$_{neg}$   \\ \cmidrule(l){2-17} 
                        & E-MLP     & 91.00          & 90.44 & \textbf{4.35} & \textbf{9.56} & 90.41          & \textbf{69.73} & 85.18 & \textbf{15.45} & \textbf{14.69} & 84.87          & 55.03          & 78.39          & 23.36          & \textbf{21.63} & 78.42          \\
                        & E-T5 \ours     & 91.00          & 71.03 & 19.97         & 22.40         & 4.63           & \textbf{69.73} & 31.73 & 38.80          & 61.80          & 16.83          & 55.03          & 29.72          & 26.28          & 56.23          & 12.54          \\
                        & I-Vanilla & 88.25          & 70.91 & 17.34         & 20.16         & \textbf{3.86}  & 63.07          & 29.81 & 34.08          & 59.42          & \textbf{11.42} & 48.08          & 25.32          & 23.69          & 55.53          & \textbf{7.59}  \\
                        & I-Iter \ours    & \textbf{91.69} & 71.76 & 19.93         & 22.23         & 5.43           & 68.23          & 33.46 & 36.87          & 59.79          & 18.96          & \textbf{56.23} & 35.21          & \textbf{21.42} & 50.98          & 17.48          \\
                        & I-Simul \ours   & 91.38          & 70.92 & 20.47         & 22.80         & 4.30           & 70.29          & 32.03 & 42.12          & 60.65          & 14.72          & 54.75          & 26.18          & 30.70          & 59.34          & 8.67           \\ \midrule
\multirow{6}{*}{Large}  & Method    & Acc            & Conf  & ECE           & CErr$_{pos}$  & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf           & ECE            & CErr$_{pos}$   & CErr$_{neg}$   \\ \cmidrule(l){2-17} 
                        & E-MLP     & 91.00          & 91.34 & \textbf{5.13} & \textbf{8.66} & 91.31          & 69.73          & 84.06 & \textbf{14.73} & \textbf{16.04} & 84.28          & 55.03          & 75.87          & \textbf{20.83} & \textbf{24.17} & 75.91          \\
                        & E-T5 \ours     & 91.00          & 70.36 & 20.65         & 23.02         & 3.40           & 69.73          & 35.23 & 38.72          & 57.70          & 18.95          & 55.03          & 27.61          & 28.30          & 58.42          & 10.50          \\
                        & I-Vanilla & 89.14          & 70.03 & 19.11         & 21.79         & \textbf{2.91}  & 68.23          & 32.70 & 38.85          & 58.35          & \textbf{13.49} & 42.52          & 21.53          & 21.80          & 55.84          & \textbf{4.79}  \\
                        & I-Iter \ours    & \textbf{92.20} & 72.66 & 19.54         & 21.66         & 5.58           & \textbf{70.67} & 33.17 & 38.49          & 60.59          & 18.13          & \textbf{55.38} & 26.91          & 28.86          & 59.90          & 10.52          \\
                        & I-Simul \ours   & 91.87          & 71.72 & 20.15         & 22.38         & 5.09           & 69.54          & 31.45 & 38.26          & 61.73          & 15.88          & 55.28          & 26.35          & 29.37          & 60.57          & 10.17          \\ \bottomrule
\end{tabular}

}
\caption{Results of T5's calibration performance with increasing dataset sizes. 
We observe a significant improvement in calibration performance when increasing the dataset size from small to middle.}

\label{tab:emergent_dev_size}
\end{table*}

==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/tab/emergent_scale.tex <==
\begin{table*}[thb]

\resizebox{\textwidth}{!}{

\begin{tabular}{@{}l|l|ccccc|ccccc|ccccc@{}}
\toprule
Model Scale               & Dataset   & \multicolumn{5}{c|}{Amazon}                                             & \multicolumn{5}{c|}{SST-5}                                                & \multicolumn{5}{c}{SemEval}                                              \\ \midrule
\multirow{6}{*}{T5-small} & Method    & Acc            & Conf  & ECE           & CErr$_{pos}$   & CErr$_{neg}$  & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$  \\ \cmidrule(l){2-17} 
                          & E-MLP     & 87.65          & 86.41 & \textbf{4.78} & \textbf{13.59} & 86.43         & \textbf{65.14} & 80.15 & \textbf{15.23} & \textbf{19.86} & 80.17          & 49.23          & 77.14 & 27.91          & \textbf{22.89} & 77.17         \\
                          & E-T5 \ours     & 87.65          & 67.80 & 19.85         & 23.71          & 7.49          & \textbf{65.14} & 28.16 & 37.29          & 64.06          & 13.63          & 49.23          & 30.45 & 19.40          & 50.65          & 12.12         \\
                          & I-Vanilla & 81.64          & 57.35 & 24.28         & 30.30          & \textbf{2.45} & 55.01          & 3.95  & 51.21          & 93.35          & \textbf{0.66}  & 44.57          & 2.17  & 42.43          & 95.53          & \textbf{0.32} \\
                          & I-Iter \ours    & 87.54          & 68.20 & 19.33         & 22.89          & 5.66          & 64.10          & 28.81 & 36.99          & 62.99          & 14.16          & 48.52          & 32.05 & \textbf{17.49} & 47.86          & 13.13         \\
                          & I-Simul \ours   & \textbf{87.66} & 68.61 & 19.05         & 22.63          & 6.35          & 64.57          & 29.59 & 37.57          & 62.38          & 14.95          & \textbf{50.38}          & 35.00 & 18.89          & 45.87          & 15.58         \\ \midrule
\multirow{6}{*}{T5-base}  & Method    & Acc            & Conf  & ECE           & CErr$_{pos}$   & CErr$_{neg}$  & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$  \\ \cmidrule(l){2-17} 
                          & E-MLP     & 91.00          & 90.44 & \textbf{4.35} & \textbf{9.56}  & 90.41         & 69.73          & 85.18 & \textbf{15.45} & \textbf{14.69} & 84.87          & 55.03          & 78.39 & 23.36          & \textbf{21.63} & 78.42         \\
                          & E-T5 \ours     & 91.00          & 71.03 & 19.97         & 22.40          & 4.63          & 69.73          & 31.73 & 38.80          & 61.80          & 16.83          & 55.03          & 29.72 & 26.28          & 56.23          & 12.54         \\
                          & I-Vanilla & 88.25          & 70.91 & 17.34         & 20.16          & \textbf{3.86} & 63.07          & 29.81 & 34.08          & 59.42          & \textbf{11.42} & 48.08          & 25.32 & 23.69          & 55.53          & \textbf{7.59} \\
                          & I-Iter \ours    & \textbf{91.69} & 71.76 & 19.93         & 22.23          & 5.43          & 68.23          & 33.46 & 36.87          & 59.79          & 18.96          & \textbf{56.23} & 35.21 & \textbf{21.42} & 50.98          & 17.48         \\
                          & I-Simul \ours   & 91.38          & 70.92 & 20.47         & 22.80          & 4.30          & \textbf{70.29} & 32.03 & 42.12          & 60.65          & 14.72          & 54.75          & 26.18 & 30.70          & 59.34          & 8.67          \\ \midrule
\multirow{6}{*}{T5-large} & Method    & Acc            & Conf  & ECE           & CErr$_{pos}$   & CErr$_{neg}$  & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$  \\ \cmidrule(l){2-17} 
                          & E-MLP     & 91.58          & 91.95 & \textbf{4.70} & \textbf{8.04}  & 91.89         & \textbf{73.85} & 83.52 & \textbf{10.24} & \textbf{16.52} & 83.61          & 56.65          & 78.26 & \textbf{21.61} & \textbf{21.74} & 78.26         \\
                          & E-T5 \ours     & 91.58          & 70.10 & 21.48         & 23.70          & 2.66          & \textbf{73.85} & 29.96 & 47.35          & 64.65          & 14.75          & 56.65          & 28.56 & 29.98          & 57.52          & 10.36         \\
                          & I-Vanilla & 88.88          & 69.42 & 19.46         & 22.12          & \textbf{1.81} & 71.79          & 28.30 & 46.83          & 65.12          & \textbf{11.55} & 49.00          & 24.66 & 25.95          & 56.30          & \textbf{6.37} \\
                          & I-Iter \ours    & 92.96          & 88.26 & 10.48         & 8.74           & 48.71         & 72.45          & 70.35 & 30.29          & 25.22          & 58.71          & \textbf{58.08} & 84.26 & 35.21          & 12.77          & 80.14         \\
                          & I-Simul \ours   & \textbf{93.34} & 74.45 & 19.39         & 20.62          & 5.43          & 73.66          & 36.92 & 45.40          & 57.27          & 20.66          & 56.87          & 40.04 & 28.43          & 44.23          & 19.29         \\ \bottomrule
\end{tabular}

}
\caption{Results of T5's calibration performance with increasing model scales.}
\label{tab:emergent_scale}
\end{table*}

==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/tab/entropy_roberta.tex <==

\begin{table*}

\resizebox{\textwidth}{!}{

\begin{tabular}{@{}ll|cccccc|cccccc@{}}
\toprule
\multicolumn{2}{c|}{ID Dataset}                                 & \multicolumn{6}{c|}{SST-2}                                                                                      & \multicolumn{6}{c}{Yahoo}                                                                                      \\ \midrule
\multicolumn{2}{c|}{OOD Dataset}                                & \multicolumn{2}{c|}{SST-2}           & \multicolumn{2}{c|}{Bookcorpus}      & \multicolumn{2}{c|}{Random Words} & \multicolumn{2}{c|}{Yahoo}           & \multicolumn{2}{c|}{Bookcorpus}      & \multicolumn{2}{c}{Random Words} \\ \midrule
\multicolumn{2}{c|}{Method}                                     & Conf  & \multicolumn{1}{c|}{Entropy} & Conf  & \multicolumn{1}{c|}{Entropy} & Conf           & Entropy          & Conf  & \multicolumn{1}{c|}{Entropy} & Conf  & \multicolumn{1}{c|}{Entropy} & Conf           & Entropy         \\ \midrule
\multicolumn{1}{l|}{\multirow{5}{*}{Unlearnable}} & Vanilla     & 98.33 & \multicolumn{1}{c|}{4.27}    & 94.85 & \multicolumn{1}{c|}{12.63}   & 96.28          & 9.97             & 90.18 & \multicolumn{1}{c|}{26.96}   & 72.17 & \multicolumn{1}{c|}{77.84}   & 78.49          & 59.14           \\
\multicolumn{1}{l|}{}                             & TS          & 93.43 & \multicolumn{1}{c|}{19.62}   & 86.41 & \multicolumn{1}{c|}{32.66}   & 87.50          & 32.46            & 71.73 & \multicolumn{1}{c|}{90.13}   & 44.01 & \multicolumn{1}{c|}{163.43}  & 50.51          & 148.65          \\
\multicolumn{1}{l|}{}                             & LS          & 87.88 & \multicolumn{1}{c|}{35.74}   & 83.30 & \multicolumn{1}{c|}{42.64}   & 82.88          & 44.11            & 82.08 & \multicolumn{1}{c|}{74.02}   & 67.53 & \multicolumn{1}{c|}{110.10}  & 74.89          & 93.55           \\
\multicolumn{1}{l|}{}                             & EDA         & 98.43 & \multicolumn{1}{c|}{3.67}    & 95.54 & \multicolumn{1}{c|}{10.79}   & 91.55          & 20.06            & 94.24 & \multicolumn{1}{c|}{15.08}   & 83.30 & \multicolumn{1}{c|}{44.77}   & 86.10          & 35.91           \\
\multicolumn{1}{l|}{}                             & Ensemble    & 98.24 & \multicolumn{1}{c|}{4.49}    & 94.65 & \multicolumn{1}{c|}{12.87}   & 93.26          & 15.98            & 91.22 & \multicolumn{1}{c|}{23.92}   & 75.10 & \multicolumn{1}{c|}{69.13}   & 80.31          & 54.06           \\ \midrule
\multicolumn{1}{l|}{\multirow{5}{*}{Learnable}}   & E-MLP       & 94.48 & \multicolumn{1}{c|}{15.99}   & 80.75 & \multicolumn{1}{c|}{36.41}   & 63.81          & 59.36            & 74.15 & \multicolumn{1}{c|}{-}       & 41.87 & \multicolumn{1}{c|}{-}       & 42.31          & -               \\
\multicolumn{1}{l|}{}                             & E-T5 \ours       & 84.79 & \multicolumn{1}{c|}{16.26}   & 63.99 & \multicolumn{1}{c|}{24.34}   & 22.84          & 27.72            & 68.71 & \multicolumn{1}{c|}{-}       & 22.70 & \multicolumn{1}{c|}{-}       & 15.20          & -               \\
\multicolumn{1}{l|}{}                             & I-Vanilla   & 84.83 & \multicolumn{1}{c|}{16.33}   & 65.34 & \multicolumn{1}{c|}{25.09}   & 23.08          & 28.39            & 69.55 & \multicolumn{1}{c|}{-}       & 24.84 & \multicolumn{1}{c|}{-}       & 17.78          & -               \\
\multicolumn{1}{l|}{}                             & I-Iter \ours & 56.89 & \multicolumn{1}{c|}{20.06}   & 62.99 & \multicolumn{1}{c|}{21.10}   & 42.25          & 30.37            & 76.16 & \multicolumn{1}{c|}{-}       & 54.33 & \multicolumn{1}{c|}{-}       & 48.54          & -               \\
\multicolumn{1}{l|}{}                             & I-Simul \ours & 75.24 & \multicolumn{1}{c|}{9.44}    & 46.51 & \multicolumn{1}{c|}{13.88}   & 8.11           & 5.44             & 64.66 & \multicolumn{1}{c|}{-}       & 19.70 & \multicolumn{1}{c|}{-}       & 19.47          & -               \\ \bottomrule
\end{tabular}
}
\caption{Results on task-irrelevant inputs with RoBERTa. We don't report the entropy results of learnable methods when Yahoo is adopted as ID dataset since the class numbers are different in unlearnable (10 original classes in Yahoo) and learnable methods (2 classes), which will result in unfair comparison.}
\label{tab:robertaentropy}
\end{table*}

==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/tab/entropy_t5.tex <==

\begin{table*}

\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}ll|cccccc|cccccc@{}}
\toprule
\multicolumn{2}{c|}{ID Dataset}                               & \multicolumn{6}{c|}{SST-2}                                                                                      & \multicolumn{6}{c}{Yahoo}                                                                                      \\ \midrule
\multicolumn{2}{c|}{OOD Dataset}                              & \multicolumn{2}{c|}{SST-2}           & \multicolumn{2}{c|}{Bookcorpus}      & \multicolumn{2}{c|}{Random Words} & \multicolumn{2}{c|}{Yahoo}           & \multicolumn{2}{c|}{Bookcorpus}      & \multicolumn{2}{c}{Random Words} \\ \midrule
\multicolumn{2}{c|}{Method}                                   & Conf  & \multicolumn{1}{c|}{Entropy} & Conf  & \multicolumn{1}{c|}{Entropy} & Conf           & Entropy          & Conf  & \multicolumn{1}{c|}{Entropy} & Conf  & \multicolumn{1}{c|}{Entropy} & Conf           & Entropy         \\ \midrule
\multicolumn{1}{l|}{\multirow{5}{*}{Unlearnable}} & Vanilla   & 98.04 & \multicolumn{1}{c|}{5.01}    & 93.38 & \multicolumn{1}{c|}{15.97}   & 84.46          & 34.95            & 82.76 & \multicolumn{1}{c|}{51.94}   & 47.62 & \multicolumn{1}{c|}{152.43}  & 56.95          & 126.54          \\
\multicolumn{1}{l|}{}                             & TS        & 93.89 & \multicolumn{1}{c|}{18.02}   & 85.07 & \multicolumn{1}{c|}{35.23}   & 72.49          & 54.69            & 75.72 & \multicolumn{1}{c|}{76.29}   & 38.43 & \multicolumn{1}{c|}{177.74}  & 47.70          & 154.00          \\
\multicolumn{1}{l|}{}                             & LS        & 88.64 & \multicolumn{1}{c|}{33.90}   & 83.65 & \multicolumn{1}{c|}{40.46}   & 72.31          & 55.30            & 74.35 & \multicolumn{1}{c|}{93.81}   & 44.29 & \multicolumn{1}{c|}{168.14}  & 54.08          & 145.94          \\
\multicolumn{1}{l|}{}                             & EDA       & 98.27 & \multicolumn{1}{c|}{4.33}    & 93.73 & \multicolumn{1}{c|}{15.45}   & 83.00          & 37.15            & 83.68 & \multicolumn{1}{c|}{46.75}   & 50.59 & \multicolumn{1}{c|}{141.92}  & 69.03          & 92.58           \\
\multicolumn{1}{l|}{}                             & Ensemble  & 97.96 & \multicolumn{1}{c|}{5.20}    & 93.21 & \multicolumn{1}{c|}{16.47}   & 82.75          & 37.87            & 82.41 & \multicolumn{1}{c|}{53.01}   & 48.29 & \multicolumn{1}{c|}{150.39}  & 55.87          & 130.57          \\ \midrule
\multicolumn{1}{l|}{\multirow{5}{*}{Learnable}}   & E-MLP     & 88.62 & \multicolumn{1}{c|}{35.37}   & 86.94 & \multicolumn{1}{c|}{38.69}   & 85.04          & 42.17            & 74.93 & \multicolumn{1}{c|}{-}       & 61.80 & \multicolumn{1}{c|}{-}       & 67.57          & -               \\
\multicolumn{1}{l|}{}                             & E-T5 \ours     & 55.96 & \multicolumn{1}{c|}{62.11}   & 56.35 & \multicolumn{1}{c|}{64.08}   & 64.02          & 60.32            & 60.29 & \multicolumn{1}{c|}{-}       & 13.64 & \multicolumn{1}{c|}{-}       & 22.56          & -               \\
\multicolumn{1}{l|}{}                             & I-Vanilla & 56.31 & \multicolumn{1}{c|}{62.13}   & 57.72 & \multicolumn{1}{c|}{63.99}   & 66.47          & 59.90            & 60.51 & \multicolumn{1}{c|}{-}       & 13.71 & \multicolumn{1}{c|}{-}       & 22.78          & -               \\
\multicolumn{1}{l|}{}                             & I-Iter \ours   & 43.43 & \multicolumn{1}{c|}{57.59}   & 43.24 & \multicolumn{1}{c|}{60.62}   & 56.07          & 61.10            & 61.35 & \multicolumn{1}{c|}{-}       & 20.62 & \multicolumn{1}{c|}{-}       & 39.08          & -               \\
\multicolumn{1}{l|}{}                             & I-Simul \ours  & 63.24 & \multicolumn{1}{c|}{10.50}   & 65.74 & \multicolumn{1}{c|}{2.25}    & 77.68          & 0.01             & 60.52 & \multicolumn{1}{c|}{-}       & 6.44  & \multicolumn{1}{c|}{-}       & 14.67          & -               \\ \bottomrule
\end{tabular}
}

\caption{Results on task-irrelevant inputs with T5. We don't report the entropy results of learnable methods when Yahoo is adopted as ID dataset since the class numbers are different in unlearnable (10 original classes in Yahoo) and learnable methods (2 classes), which will result in unfair comparison.}
\label{tab:entropyt5}
\end{table*}

==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/tab/hard2easyroberta.tex <==
\begin{table*}[t!]
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}l|ll|ccccc|ccccc|ccccc@{}}
\toprule
\multirow{12}{*}{Dynasent} & \multicolumn{2}{l|}{Dataset}                                  & \multicolumn{5}{c|}{Dynasent}                                           & \multicolumn{5}{c|}{Amazon}                                             & \multicolumn{5}{c}{DSC}                                                  \\ \cmidrule(l){2-18} 
                           & \multicolumn{2}{l|}{Method}                                   & Acc            & Conf  & ECE           & CErr$_{pos}$  & CErr$_{neg}$   & Acc            & Conf  & ECE           & CErr$_{pos}$  & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$  & CErr$_{neg}$   \\ \cmidrule(l){2-18} 
                           & \multicolumn{1}{l|}{\multirow{5}{*}{Unlearnable}} & Vanilla   & \textbf{78.61} & 94.56 & 17.10         & \textbf{3.56} & 88.06          & 85.47          & 97.84 & 12.48         & 1.18          & 92.08          & 87.93          & 97.23 & 9.30           & 1.74          & 89.70          \\
                           & \multicolumn{1}{l|}{}                             & TS        & \textbf{78.61} & 77.47 & \textbf{0.95} & 19.47         & 66.96          & 85.47          & 86.61 & \textbf{2.54} & 11.24         & 74.11          & 87.93          & 85.09 & 2.99           & 12.84         & 70.03          \\
                           & \multicolumn{1}{l|}{}                             & LS        & 76.48          & 85.95 & 9.46          & 12.37         & 80.47          & \textbf{85.85} & 89.34 & 7.39          & 9.53          & 82.53          & \textbf{87.15} & 88.19 & 5.46           & 10.71         & 80.75          \\
                           & \multicolumn{1}{l|}{}                             & EDA       & 76.97          & 95.65 & 18.74         & 2.92          & 90.85          & 84.12          & 97.92 & 13.81         & 1.08          & 92.64          & 85.53          & 97.13 & 11.62          & 1.64          & 89.87          \\
                           & \multicolumn{1}{l|}{}                             & Ensemble  & 77.67          & 94.85 & 17.22         & 3.44          & 88.89          & 85.37          & 97.88 & 12.52         & \textbf{1.12} & 92.11          & 86.69          & 97.11 & 10.43          & \textbf{1.76} & 89.77          \\ \cmidrule(l){2-18} 
                           & \multicolumn{1}{l|}{\multirow{5}{*}{Learnable}}   & E-MLP     & \textbf{78.61} & 71.06 & 19.59         & 28.81         & 70.59          & 85.47          & 85.74 & 12.10         & 14.25         & 85.69          & 87.93          & 79.37 & \textbf{14.46} & 20.61         & 79.25          \\
                           & \multicolumn{1}{l|}{}                             & E-T5 \ours     & \textbf{78.61} & 64.94 & 23.76         & 26.76         & \textbf{34.43} & 85.47          & 85.53 & 13.23         & 9.45          & \textbf{56.03} & 87.93          & 81.72 & 14.91          & 13.50         & \textbf{49.71} \\
                           & \multicolumn{1}{l|}{}                             & I-Vanilla & 77.38          & 66.71 & 22.76         & 24.92         & 38.06          & 83.85          & 85.80 & 12.18         & 7.99          & 53.56          & 87.10          & 82.30 & 14.25          & 12.89         & 49.77          \\
                           & \multicolumn{1}{l|}{}                             & I-Iter \ours   & 77.89          & 64.17 & 21.98         & 28.43         & 38.09          & 84.49          & 87.49 & 10.00         & 7.47          & 60.06          & 87.05          & 82.83 & 12.14          & 12.86         & 53.81          \\
                           & \multicolumn{1}{l|}{}                             & I-Simul \ours  & 78.63          & 65.00 & 25.56         & 27.08         & 35.84          & 83.65          & 79.79 & 15.36         & 13.28         & 44.38          & 85.79          & 77.29 & 17.78          & 16.91         & 42.30          \\ \bottomrule
\end{tabular}
}
\caption{Results of RoBERTa's calibration performance under hard-to-easy distribution shifts.}

\label{tab:hard2easy-roberta}
\end{table*} 

==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/tab/hard2easyt5.tex <==
\begin{table*}[]

\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}l|ll|ccccc|ccccc|ccccc@{}}
\toprule
\multirow{12}{*}{Dynasent} & \multicolumn{2}{l|}{Dataset}                                  & \multicolumn{5}{c|}{Dynasent}                                           & \multicolumn{5}{c|}{Amazon}                                             & \multicolumn{5}{c}{DSC}                                                 \\ \cmidrule(l){2-18} 
                           & \multicolumn{2}{l|}{Method}                                   & Acc            & Conf  & ECE           & CErr$_{pos}$  & CErr$_{neg}$   & Acc            & Conf  & ECE           & CErr$_{pos}$  & CErr$_{neg}$   & Acc            & Conf  & ECE           & CErr$_{pos}$  & CErr$_{neg}$   \\ \cmidrule(l){2-18} 
                           & \multicolumn{1}{l|}{\multirow{5}{*}{Unlearnable}} & Vanilla   & 78.45          & 86.83 & 8.38          & 9.94          & 75.07          & 86.57          & 95.28 & 8.71          & 3.44          & 87.02          & \textbf{90.00} & 94.40 & 4.48          & 4.10          & 80.85          \\
                           & \multicolumn{1}{l|}{}                             & TS        & 78.45          & 79.10 & \textbf{1.02} & 17.37         & 66.27          & 86.57          & 89.92 & 3.36          & 8.59          & 80.31          & \textbf{90.00} & 89.26 & \textbf{0.78} & 8.90          & 72.68          \\
                           & \multicolumn{1}{l|}{}                             & LS        & \textbf{78.47} & 78.22 & 3.64          & 18.89         & 67.69          & 86.55          & 85.48 & 3.42          & 13.35         & 77.91          & 89.75          & 84.61 & 5.31          & 13.95         & 72.02          \\
                           & \multicolumn{1}{l|}{}                             & EDA       & 76.30          & 89.20 & 12.91         & \textbf{7.76} & 79.44          & \textbf{87.19} & 97.07 & 9.88          & \textbf{1.75} & 89.04          & 88.05          & 95.50 & 7.45          & \textbf{2.81} & 83.03          \\
                           & \multicolumn{1}{l|}{}                             & Ensemble  & 78.18          & 86.76 & 8.58          & 9.89          & 74.75          & 86.37          & 95.02 & 8.66          & 3.71          & 86.99          & 89.74          & 94.27 & 4.56          & 4.17          & 80.67          \\ \cmidrule(l){2-18} 
                           & \multicolumn{1}{l|}{\multirow{5}{*}{Learnable}}   & E-MLP     & 78.45          & 78.99 & 4.45          & 21.05         & 79.11          & 86.57          & 83.15 & \textbf{2.92} & 16.85         & 83.14          & \textbf{90.00} & 82.53 & 7.17          & 17.48         & 82.63          \\
                           & \multicolumn{1}{l|}{}                             & E-T5 \ours     & 78.45          & 61.63 & 18.26         & 33.00         & 42.07          & 86.57          & 89.99 & 6.51          & 6.94          & 71.00          & \textbf{90.00} & 86.14 & 6.19          & 11.03         & 61.60          \\
                           & \multicolumn{1}{l|}{}                             & I-Vanilla & \textbf{78.47} & 61.95 & 17.91         & 32.77         & 42.72          & 84.44          & 89.89 & 6.52          & 6.18          & 68.52          & 88.84          & 86.15 & 5.76          & 10.77         & 61.69          \\
                           & \multicolumn{1}{l|}{}                             & I-Iter \ours   & 77.92          & 61.45 & 16.47         & 33.26         & 42.78          & 86.03          & 86.92 & 2.99          & 9.99          & \textbf{67.91} & 89.45          & 84.72 & 4.88          & 12.54         & 61.55          \\
                           & \multicolumn{1}{l|}{}                             & I-Simul \ours  & 78.13          & 66.36 & 24.59         & 25.51         & \textbf{37.34} & 85.67          & 91.26 & 13.29         & 5.28          & 70.59          & 88.61          & 87.83 & 12.46         & 8.41          & \textbf{58.61} \\ \bottomrule
\end{tabular}
}

\caption{Results T5's calibration performance under hard-to-easy distribution shifts.}
% Results of T5’s calibration performance under standard distribution shifts
\label{tab:hard2easyt5}
\vspace{-10pt}
\end{table*}

==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/tab/methods_shift_roberta.tex <==
\begin{table*}[t!]
\centering

\resizebox{\textwidth}{!}{
\begin{tabular}{@{}l|ll|ccccc|ccccc|ccccc@{}}
\toprule
\multirow{12}{*}{MNLI}   & \multicolumn{2}{l|}{Dataset}                                  & \multicolumn{5}{c|}{MNLI}                                               & \multicolumn{5}{c|}{HANS}                                                & \multicolumn{5}{c}{ANLI}                                                 \\ \cmidrule(l){2-18} 
                         & \multicolumn{2}{l|}{Method}                                   & Acc            & Conf  & ECE           & CErr$_{pos}$  & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$  & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$  & CErr$_{neg}$   \\ \cmidrule(l){2-18} 
                         & \multicolumn{1}{l|}{\multirow{5}{*}{Unlearnable}} & Vanilla   & 85.90          & 96.24 & 9.50          & 2.40          & 87.36          & 54.17          & 95.09 & 39.68          & 2.71          & 92.36          & 29.78          & 90.94 & 61.14          & 11.28         & 91.90          \\
                         & \multicolumn{1}{l|}{}                             & TS        & 85.90          & 86.65 & \textbf{0.90} & 11.09         & 71.84          & 54.17          & 82.15 & 26.74          & 15.43         & 79.16          & 29.78          & 75.57 & 45.57          & 27.32         & 76.80          \\
                         & \multicolumn{1}{l|}{}                             & LS        & 86.28          & 86.88 & 4.43          & 11.92         & 79.31          & 55.59          & 86.96 & 31.37          & 11.47         & 85.00          & 29.25          & 81.59 & 52.37          & 20.23         & 82.34          \\
                         & \multicolumn{1}{l|}{}                             & EDA       & 85.99          & 97.07 & 11.09         & \textbf{1.78} & 90.05          & \textbf{58.24} & 96.87 & 38.63          & \textbf{1.91} & 95.16          & \textbf{31.34} & 92.00 & 60.66          & \textbf{8.81} & 92.38          \\
                         & \multicolumn{1}{l|}{}                             & Ensemble  & 86.60          & 96.32 & 9.74          & 2.37          & 87.90          & 56.09          & 96.44 & 40.35          & 2.00          & 94.45          & 30.06          & 90.47 & 60.46          & 11.38         & 91.26          \\ \cmidrule(l){2-18} 
                         & \multicolumn{1}{l|}{\multirow{5}{*}{Learnable}}   & E-MLP     & 85.90          & 85.82 & 13.73         & 14.16         & 85.67          & 54.17          & 81.92 & 29.36          & 17.87         & 81.66          & 29.78          & 81.49 & 51.71          & 18.88         & 81.65          \\
                         & \multicolumn{1}{l|}{}                             & E-T5 \ours     & 85.90          & 74.37 & 18.51         & 18.93         & 33.58          & 54.17          & 74.47 & 28.79          & 10.10         & 56.23          & 29.78          & 35.21 & 45.46          & 74.72         & 39.43          \\
                         & \multicolumn{1}{l|}{}                             & I-Vanilla & 85.76          & 75.23 & 18.25         & 18.32         & 36.45          & 57.28          & 77.14 & 32.26          & 13.23         & 64.23          & 28.63          & 37.14 & 44.78          & 71.91         & 40.77          \\
                         & \multicolumn{1}{l|}{}                             & I-Iter \ours    & \textbf{86.63} & 60.04 & 26.59         & 33.85         & \textbf{20.41} & 53.70          & 57.77 & \textbf{21.70} & 29.34         & \textbf{42.82} & 31.06          & 21.29 & \textbf{31.88} & 83.71         & \textbf{23.55} \\
                         & \multicolumn{1}{l|}{}                             & I-Simul \ours   & 86.46          & 74.81 & 18.91         & 18.49         & 32.01          & 56.65          & 75.84 & 33.83          & 13.79         & 62.28          & 29.16          & 38.67 & 45.44          & 66.86         & 40.95          \\ \midrule
\multirow{12}{*}{Amazon} & \multicolumn{2}{l|}{Dataset}                                  & \multicolumn{5}{c|}{Amazon}                                             & \multicolumn{5}{c|}{SST-5}                                               & \multicolumn{5}{c}{SemEval}                                              \\ \cmidrule(l){2-18} 
                         & \multicolumn{2}{l|}{Method}                                   & Acc            & Conf  & ECE           & CErr$_{pos}$  & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$  & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$  & CErr$_{neg}$   \\ \cmidrule(l){2-18} 
                         & \multicolumn{1}{l|}{\multirow{5}{*}{Unlearnable}} & Vanilla   & 90.90          & 98.17 & 7.28          & 1.09          & 90.84          & \textbf{70.29} & 94.29 & 24.05          & 3.95          & 90.14          & 56.02          & 90.45 & 34.43          & 7.05          & 87.26          \\
                         & \multicolumn{1}{l|}{}                             & TS        & 90.90          & 89.66 & \textbf{2.02} & 8.73          & 73.58          & \textbf{70.29} & 78.15 & \textbf{7.91}  & 18.42         & 70.04          & 56.02          & 70.34 & \textbf{14.32} & 25.98         & 65.65          \\
                         & \multicolumn{1}{l|}{}                             & LS        & 91.89          & 88.50 & 6.71          & 10.64         & 78.83          & 69.92          & 84.01 & 14.20          & 14.38         & 80.28          & 55.17          & 81.64 & 26.47          & 15.46         & 78.08          \\
                         & \multicolumn{1}{l|}{}                             & EDA       & \textbf{92.39} & 98.34 & 5.95          & \textbf{0.92} & 89.46          & 66.64          & 93.98 & 27.34          & \textbf{3.82} & 89.57          & \textbf{57.05} & 93.45 & 36.43          & \textbf{4.37} & 90.56          \\
                         & \multicolumn{1}{l|}{}                             & Ensemble  & 91.69          & 98.19 & 6.50          & 1.06          & 89.93          & 69.56          & 93.67 & 24.22          & 4.24          & 88.93          & 55.94          & 90.14 & 34.23          & 7.19          & 86.76          \\ \cmidrule(l){2-18} 
                         & \multicolumn{1}{l|}{\multirow{5}{*}{Learnable}}   & E-MLP     & 90.90          & 95.08 & 9.14          & 4.94          & 95.34          & \textbf{70.29} & 83.57 & 22.22          & 16.18         & 82.99          & 56.02          & 77.12 & 25.42          & 22.49         & 76.63          \\
                         & \multicolumn{1}{l|}{}                             & E-T5 \ours     & 90.90          & 71.97 & 19.27         & 21.20         & 3.72           & \textbf{70.29} & 32.10 & 45.94          & 61.74         & 17.53          & 56.02          & 23.64 & 36.13          & 64.58         & 8.63           \\
                         & \multicolumn{1}{l|}{}                             & I-Vanilla & 88.00          & 71.60 & 17.13         & 19.18         & 3.97           & 64.85          & 26.74 & 46.32          & 65.75         & \textbf{12.86} & 44.43          & 17.51 & 31.05          & 66.92         & \textbf{5.07}  \\
                         & \multicolumn{1}{l|}{}                             & I-Iter \ours    & 90.11          & 71.34 & 18.88         & 21.18         & \textbf{3.24}  & 66.54          & 34.13 & 41.70          & 58.17         & 18.82          & 53.28          & 34.05 & 27.10          & 48.25         & 13.86          \\
                         & \multicolumn{1}{l|}{}                             & I-Simul \ours   & 90.60          & 71.07 & 19.80         & 21.91         & 3.41           & 69.35          & 33.96 & 44.16          & 58.75         & 17.46          & 53.50          & 24.20 & 33.35          & 61.15         & 7.36           \\ \midrule
\multirow{12}{*}{Civil}  & \multicolumn{2}{l|}{Dataset}                                  & \multicolumn{5}{c|}{Civil}                                              & \multicolumn{5}{c|}{Hate Speech}                                         & \multicolumn{5}{c}{Implicit Hate}                                        \\ \cmidrule(l){2-18} 
                         & \multicolumn{2}{l|}{Method}                                   & Acc            & Conf  & ECE           & CErr$_{pos}$  & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$  & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$  & CErr$_{neg}$   \\ \cmidrule(l){2-18} 
                         & \multicolumn{1}{l|}{\multirow{5}{*}{Unlearnable}} & Vanilla   & 86.94          & 98.15 & 10.09         & \textbf{1.14} & 92.91          & 76.99          & 98.22 & 21.94          & \textbf{1.22} & 96.41          & \textbf{62.88} & 96.37 & 32.02          & 2.88          & 95.00          \\
                         & \multicolumn{1}{l|}{}                             & TS        & 86.94          & 90.94 & \textbf{2.88} & 7.29          & 77.87          & 76.99          & 89.70 & 13.34          & 8.58          & 84.16          & \textbf{62.88} & 85.50 & \textbf{21.15} & 12.72         & 82.28          \\
                         & \multicolumn{1}{l|}{}                             & LS        & \textbf{87.91} & 87.73 & 9.52          & 11.79         & 84.24          & \textbf{78.45} & 88.31 & \textbf{10.86} & 11.48         & 87.54          & 62.58          & 86.79 & 24.21          & 12.82         & 86.13          \\
                         & \multicolumn{1}{l|}{}                             & EDA       & 83.61          & 97.01 & 13.40         & 2.08          & 92.35          & 77.82          & 97.28 & 19.65          & 2.30          & 95.82          & 61.53          & 96.68 & 35.14          & \textbf{2.71} & 95.70          \\
                         & \multicolumn{1}{l|}{}                             & Ensemble  & 86.45          & 97.96 & 11.52         & 1.29          & 93.16          & 76.32          & 97.58 & 21.28          & 1.75          & 95.41          & 62.77          & 96.19 & 33.42          & 3.08          & 94.97          \\ \cmidrule(l){2-18} 
                         & \multicolumn{1}{l|}{\multirow{5}{*}{Learnable}}   & E-MLP     & 86.94          & 91.93 & 12.24         & 8.09          & 92.01          & 76.99          & 88.52 & 19.66          & 11.62         & 88.98          & \textbf{62.88} & 83.08 & 25.45          & 17.15         & 83.47          \\
                         & \multicolumn{1}{l|}{}                             & E-T5 \ours     & 86.94          & 70.97 & 15.99         & 18.62         & 1.68           & 76.99          & 46.28 & 48.83          & 52.25         & 41.37          & \textbf{62.88} & 30.90 & 41.57          & 59.84         & 15.20          \\
                         & \multicolumn{1}{l|}{}                             & I-Vanilla & 77.92          & 69.06 & 8.92          & 11.60         & \textbf{0.83}  & 76.99          & 45.25 & 49.59          & 53.24         & \textbf{40.21} & 58.12          & 29.51 & 38.32          & 58.58         & \textbf{13.00} \\
                         & \multicolumn{1}{l|}{}                             & I-Iter \ours    & 85.40          & 75.36 & 10.31         & 12.18         & 2.48           & 76.15          & 50.43 & 49.62          & 50.02         & 51.84          & 60.59          & 34.15 & 38.04          & 54.50         & 16.69          \\
                         & \multicolumn{1}{l|}{}                             & I-Simul \ours   & 87.25          & 70.69 & 16.65         & 19.22         & 1.71           & 78.24          & 45.86 & 50.64          & 53.36         & 43.03          & 62.56          & 29.60 & 41.56          & 60.57         & 13.17          \\ \bottomrule
\end{tabular}
}
\caption{Results of RoBERTa's calibration performance under standard distribution shifts.}
% Results of T5’s calibration performance under standard distribution shifts
\label{tab:roberta-shift}
\end{table*}







==> A Close Look into the Calibration of Pre-trained Language Models --- ACL/tab/methods_shift_t5.tex <==
\begin{table*}[thb]
\centering
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{@{}l|ll|ccccc|ccccc|ccccc@{}}
\toprule
\multirow{12}{*}{MNLI}   & \multicolumn{2}{l|}{Dataset}                                  & \multicolumn{5}{c|}{MNLI}                                               & \multicolumn{5}{c|}{HANS}                                                & \multicolumn{5}{c}{ANLI}                                                  \\ \cmidrule(l){2-18} 
                         & \multicolumn{2}{l|}{Method}                                   & Acc            & Conf  & ECE           & CErr$_{pos}$  & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$  & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   \\ \cmidrule(l){2-18} 
                         & \multicolumn{1}{l|}{\multirow{5}{*}{Unlearnable}} & Vanilla   & 86.50          & 94.85 & 8.35          & 3.47          & 84.12          & 55.06          & 92.36 & 37.30          & 5.96          & 90.30          & 31.31          & 85.58 & 54.27          & 16.22          & 86.41          \\
                         & \multicolumn{1}{l|}{}                             & TS        & 86.50          & 89.22 & \textbf{2.75} & 8.44          & 74.22          & 55.06          & 83.99 & 28.93          & 14.36         & 81.97          & 31.31          & 75.48 & 44.17          & 26.87          & 76.56          \\
                         & \multicolumn{1}{l|}{}                             & LS        & 86.19          & 85.53 & 3.41          & 13.06         & 76.74          & 56.94          & 83.74 & \textbf{26.80} & 16.19         & 83.64          & 30.50          & 77.71 & 47.21          & 23.77          & 78.36          \\
                         & \multicolumn{1}{l|}{}                             & EDA       & 86.29          & 95.44 & 9.15          & \textbf{3.06} & 86.01          & 52.73          & 92.24 & 39.50          & \textbf{4.61} & 88.72          & 30.34          & 87.45 & 57.11          & \textbf{13.86} & 88.03          \\
                         & \multicolumn{1}{l|}{}                             & Ensemble  & \textbf{86.54} & 94.82 & 8.28          & 3.53          & 84.22          & 56.52          & 91.90 & 35.38          & 6.72          & 90.15          & \textbf{31.41} & 85.49 & 54.09          & 16.49          & 86.40          \\ \cmidrule(l){2-18} 
                         & \multicolumn{1}{l|}{\multirow{5}{*}{Learnable}}   & E-MLP     & 86.50          & 89.28 & 5.52          & 10.69         & 89.10          & 55.06          & 87.38 & 32.34          & 12.59         & 87.34          & 31.31          & 81.65 & 50.74          & 18.39          & 81.66          \\
                         & \multicolumn{1}{l|}{}                             & E-T5 \ours     & 86.50          & 79.43 & 12.24         & 15.35         & 45.84          & 55.06          & 78.74 & 35.30          & 19.11         & 75.97          & 31.31          & 41.67 & 38.68          & 65.84          & 45.11          \\
                         & \multicolumn{1}{l|}{}                             & I-Vanilla & 85.58          & 78.40 & 12.45         & 15.69         & 43.33          & 53.55          & 68.34 & 33.38          & 27.48         & \textbf{63.53} & \textbf{31.41} & 40.92 & 38.30          & 65.43          & 43.82          \\
                         & \multicolumn{1}{l|}{}                             & I-Iter \ours   & 86.30          & 70.86 & 15.49         & 24.07         & 38.95          & 57.12          & 74.92 & 28.39          & 22.16         & 71.02          & 30.69          & 37.02 & \textbf{28.37} & 68.84          & \textbf{39.62} \\
                         & \multicolumn{1}{l|}{}                             & I-Simul \ours   & 86.53          & 76.50 & 17.65         & 17.15         & \textbf{35.64} & \textbf{57.15} & 80.26 & 38.64          & 15.85         & 75.08          & 30.66          & 38.65 & 46.06          & 68.40          & 41.76          \\ \midrule
\multirow{12}{*}{Amazon} & \multicolumn{2}{l|}{Dataset}                                  & \multicolumn{5}{c|}{Amazon}                                             & \multicolumn{5}{c|}{SST-5}                                               & \multicolumn{5}{c}{SemEval}                                               \\ \cmidrule(l){2-18} 
                         & \multicolumn{2}{l|}{Method}                                   & Acc            & Conf  & ECE           & CErr$_{pos}$  & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$  & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   \\ \cmidrule(l){2-18} 
                         & \multicolumn{1}{l|}{\multirow{5}{*}{Unlearnable}} & Vanilla   & 91.00          & 95.65 & 4.86          & 2.97          & 82.05          & \textbf{69.73} & 82.78 & 13.52          & 12.30         & 71.72          & 55.03          & 76.83 & 21.75          & 17.54          & 69.94          \\
                         & \multicolumn{1}{l|}{}                             & TS        & 91.00          & 90.50 & \textbf{1.39} & 7.74          & 73.20          & \textbf{69.73} & 71.98 & \textbf{4.94}  & 23.01         & 60.69          & 55.03          & 65.45 & \textbf{10.37} & 29.14          & 58.83          \\
                         & \multicolumn{1}{l|}{}                             & LS        & 91.25          & 85.75 & 6.78          & 13.14         & 74.09          & 70.67          & 73.50 & 5.55           & 22.53         & 63.95          & 53.57          & 69.79 & 16.23          & 25.65          & 64.53          \\
                         & \multicolumn{1}{l|}{}                             & EDA       & 92.00          & 96.29 & 4.29          & \textbf{2.51} & 82.46          & 67.67          & 87.58 & 20.20          & \textbf{7.97} & 78.27          & \textbf{57.27} & 83.11 & 25.96          & \textbf{11.87} & 76.40          \\
                         & \multicolumn{1}{l|}{}                             & Ensemble  & 91.57          & 95.78 & 4.21          & 2.88          & 81.14          & 69.35          & 83.00 & 13.66          & 12.13         & 72.00          & 56.34          & 77.81 & 21.47          & 16.52          & 70.49          \\ \cmidrule(l){2-18} 
                         & \multicolumn{1}{l|}{\multirow{5}{*}{Learnable}}   & E-MLP     & 91.00          & 91.34 & 5.13          & 8.66          & 91.31          & \textbf{69.73} & 84.06 & 14.73          & 16.04         & 84.28          & 55.03          & 75.87 & 20.83          & 24.17          & 75.91          \\
                         & \multicolumn{1}{l|}{}                             & E-T5 \ours     & 91.00          & 70.36 & 20.65         & 23.02         & 3.40           & \textbf{69.73} & 35.23 & 38.72          & 57.70         & 18.95          & 55.03          & 27.61 & 28.30          & 58.42          & 10.50          \\
                         & \multicolumn{1}{l|}{}                             & I-Vanilla & 89.14          & 70.03 & 19.11         & 21.79         & \textbf{2.91}  & 68.23          & 32.70 & 38.85          & 58.35         & \textbf{13.49} & 42.52          & 21.53 & 21.80          & 55.84          & \textbf{4.79}  \\
                         & \multicolumn{1}{l|}{}                             & I-Iter \ours    & \textbf{92.20} & 72.66 & 19.54         & 21.66         & 5.58           & 70.67          & 33.17 & 38.49          & 60.59         & 18.13          & 55.38          & 26.91 & 28.86          & 59.90          & 10.52          \\
                         & \multicolumn{1}{l|}{}                             & I-Simul \ours   & 91.87          & 71.72 & 20.15         & 22.38         & 5.09           & 69.54          & 31.45 & 38.26          & 61.73         & 15.88          & 55.28          & 26.35 & 29.37          & 60.57          & 10.17          \\ \midrule
\multirow{12}{*}{Civil}  & \multicolumn{2}{l|}{Dataset}                                  & \multicolumn{5}{c|}{Civil}                                              & \multicolumn{5}{c|}{Hate Speech}                                         & \multicolumn{5}{c}{Implicit Hate}                                         \\ \cmidrule(l){2-18} 
                         & \multicolumn{2}{l|}{Method}                                   & Acc            & Conf  & ECE           & CErr$_{pos}$  & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$  & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   \\ \cmidrule(l){2-18} 
                         & \multicolumn{1}{l|}{\multirow{5}{*}{Unlearnable}} & Vanilla   & 86.08          & 94.23 & 7.74          & 3.88          & 82.12          & 75.52          & 92.54 & 17.23          & 5.88          & 87.72          & 60.64          & 89.68 & 28.83          & 8.62           & 87.04          \\
                         & \multicolumn{1}{l|}{}                             & TS        & 86.08          & 89.65 & \textbf{3.16} & 7.79          & 73.27          & 75.52          & 86.29 & 11.13 & 11.60         & 79.84          & 60.64          & 82.24 & 21.38          & 15.49          & 78.71          \\
                         & \multicolumn{1}{l|}{}                             & LS        & 86.30          & 84.93 & 5.29          & 13.62         & 75.78          & 74.48          & 83.51 & \textbf{9.03}  & 14.65         & 78.15          & 60.64          & 81.19 & \textbf{20.55} & 17.36          & 78.95          \\
                         & \multicolumn{1}{l|}{}                             & EDA       & 86.87          & 95.46 & 8.59          & \textbf{3.09} & 85.83          & 73.64          & 95.20 & 21.56          & \textbf{3.57} & 91.75          & \textbf{61.95} & 92.92 & 30.97          & \textbf{5.78}  & 90.80          \\
                         & \multicolumn{1}{l|}{}                             & Ensemble  & 86.04          & 94.51 & 8.46          & 3.65          & 83.10          & 75.36          & 93.57 & 18.80          & 5.04          & 89.35          & 60.83          & 90.98 & 30.14          & 7.50           & 88.62          \\ \cmidrule(l){2-18} 
                         & \multicolumn{1}{l|}{\multirow{5}{*}{Learnable}}   & E-MLP     & 86.08          & 90.61 & 4.52          & 9.40          & 90.62          & 75.52          & 88.93 & 13.41          & 11.13         & 89.10          & 60.64          & 87.41 & 26.78          & 12.59          & 87.42          \\
                         & \multicolumn{1}{l|}{}                             & E-T5 \ours     & 86.08          & 66.22 & 19.87         & 23.24         & 0.99           & 75.52          & 41.80 & 46.42          & 55.51         & 33.51          & 60.64          & 25.28 & 40.27          & 64.82          & 10.02          \\
                         & \multicolumn{1}{l|}{}                             & I-Vanilla & 75.31          & 63.39 & 11.92         & 15.95         & \textbf{0.35}  & \textbf{75.73} & 39.32 & 48.19          & 57.19         & \textbf{28.43} & 56.39          & 22.68 & 38.30          & 65.48          & \textbf{7.38}  \\
                         & \multicolumn{1}{l|}{}                             & I-Iter \ours    & 86.58          & 69.04 & 17.53         & 20.50         & 1.61           & 74.06          & 45.69 & 44.92          & 52.14         & 39.52          & 61.29          & 29.05 & 38.67          & 60.89          & 13.11          \\
                         & \multicolumn{1}{l|}{}                             & I-Simul \ours   & \textbf{87.06} & 70.69 & 16.55         & 19.04         & 1.62           & 73.01          & 46.63 & 46.34          & 50.30         & 38.31          & 61.14          & 30.50 & 40.17          & 58.65          & 13.44          \\ \bottomrule
\end{tabular}
}
\caption{Results of T5's calibration performance under standard distribution shifts. We observe that learnable methods can significantly mitigate the overconfidence issue.}
\vspace{-10pt}
\label{tab:t5-shift}
\end{table*}







==> fig_latex/params_t5_soft.tex <==

\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim=0 0 0 0, clip, width=\textwidth]{figures/delta-soft-t5-sst2.pdf}
         \label{fig:soft-t5-sst2}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim=0 0 0 0, clip,width=\textwidth]{figures/delta-soft-t5-mnli.pdf}
         \label{fig:soft-t5-mnli}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[trim=0 6 0 10, clip,width=\textwidth]{figures/delta-soft-t5-yahoo_answers_topics.pdf}
         \label{fig:soft-t5-yahoo}
     \end{subfigure}
     
    \vspace{-10pt}
     \begin{subfigure}[b]{0.6\textwidth}
         \centering
         \includegraphics[width=0.95\textwidth]{figures/legend.pdf}
        %  \label{fig:kshots-t5-yahoo}
     \end{subfigure}
        \vspace{-2pt}
        \caption{Results of tunable parameters with T5 (soft prompt).}
        \label{fig:soft-t5}
\end{figure*}



==> tab/emergent.tex <==
\begin{table*}[]
\caption{Results on the emergent calibration of T5 with increasing dataset sizes.}

\resizebox{\textwidth}{!}{

\begin{tabular}{@{}l|l|ccccc|ccccc|ccccc@{}}
\toprule
Dataset Size              & Dataset     & \multicolumn{5}{c|}{Amazon}                                               & \multicolumn{5}{c|}{SST-5}                                                & \multicolumn{5}{c}{SemEval}                                                        \\ \midrule
\multirow{6}{*}{Small}    & Method      & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf           & ECE            & CErr$_{pos}$   & CErr$_{neg}$   \\ \cmidrule(l){2-17} 
                          & E-MLP       & 89.19          & 90.27 & 9.13           & \textbf{9.13}  & 85.30          & \textbf{67.67} & 84.41 & \textbf{18.54} & 14.93          & 83.01          & 55.02          & 82.55          & \textbf{27.85} & \textbf{16.43} & 81.30          \\
                          & E-T5        & 89.19          & 78.74 & \textbf{8.81}  & 11.41          & 31.68          & \textbf{67.67} & 79.97 & 25.61          & 14.36          & 69.96          & 55.02          & 56.08          & 31.55          & 40.78          & 52.11          \\
                          & I-Vanilla   & 88.87          & 78.15 & 9.18           & 12.02          & 30.66          & 65.98          & 75.80 & 26.17          & 18.35          & 65.82          & 55.85          & 54.67          & 31.24          & 41.76          & 50.02          \\
                          & I-Iterative & 90.04          & 80.20 & 10.23          & 10.70          & 45.30          & 66.54          & 86.12 & 24.57          & \textbf{10.60} & 80.07          & \textbf{56.40} & 62.44          & 27.98          & 35.61          & 59.53          \\
                          & I-Multitask & \textbf{90.23} & 78.22 & 8.98           & 10.02          & \textbf{21.84} & 67.10          & 56.76 & 26.16          & 31.65          & \textbf{38.75} & 55.87          & 45.78          & 37.04          & 49.90          & \textbf{39.48} \\ \midrule
\multirow{6}{*}{Middle}   & Method      & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf           & ECE            & CErr$_{pos}$   & CErr$_{neg}$   \\ \cmidrule(l){2-17} 
                          & E-MLP       & 89.19          & 89.82 & \textbf{6.92}  & \textbf{8.83}  & 78.70          & 67.67          & 81.30 & \textbf{15.72} & \textbf{17.30} & 78.37          & 55.02          & 79.01          & \textbf{24.05} & \textbf{19.45} & 77.13          \\
                          & E-T5        & 89.19          & 68.57 & 10.94          & 13.77          & 2.56           & 67.67          & 28.37 & 30.89          & 54.59          & 9.20           & 55.02          & 15.76          & 43.77          & 77.17          & 6.56           \\
                          & I-Vanilla   & 87.31          & 67.79 & 12.94          & 15.87          & \textbf{2.50}  & \textbf{65.51} & 24.90 & 33.68          & 59.76          & 6.96           & 51.50          & 15.26          & 47.71          & 78.96          & 6.62           \\
                          & I-Iterative & \textbf{90.65} & 69.70 & 9.82           & 12.20          & 3.28           & 67.10          & 20.65 & 32.25          & 64.03          & \textbf{5.01}  & \textbf{55.33} & \textbf{9.79}  & 44.08          & 85.07          & \textbf{4.25}  \\
                          & I-Multitask & 90.21          & 69.35 & 9.84           & 12.48          & 2.81           & 67.48          & 28.73 & 31.28          & 54.11          & 7.49           & \textbf{54.93} & 17.34          & 44.74          & 75.11          & 6.89           \\ \midrule
\multirow{6}{*}{Large}    & Method      & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf           & ECE            & CErr$_{pos}$   & CErr$_{neg}$   \\ \cmidrule(l){2-17} 
                          & E-MLP       & 89.19          & 89.95 & \textbf{5.34}  & \textbf{8.38}  & 76.06          & 67.76          & 79.66 & \textbf{14.11} & \textbf{18.61} & 76.03          & 55.03          & 78.22          & \textbf{23.13} & \textbf{19.94} & 75.96          \\
                          & E-T5        & 89.19          & 69.06 & 11.05          & 13.81          & \textbf{2.76}  & 67.76          & 26.04 & 30.98          & 57.08          & 6.54           & 55.03          & 12.85          & 44.42          & 80.71          & 4.99           \\
                          & I-Vanilla   & 88.52          & 69.48 & 11.66          & 14.40          & 3.05           & \textbf{68.13} & 24.56 & 30.75          & 58.11          & \textbf{5.65}  & 47.73          & 12.05          & 52.10          & 83.63          & 4.98           \\
                          & I-Iterative & \textbf{91.09} & 69.27 & 9.40           & 12.04          & 3.60           & 66.82          & 25.01 & 31.65          & 59.16          & 7.38           & 55.03          & 9.28           & 44.90          & 85.61          & \textbf{3.71}  \\
                          & I-Multitask & 90.21          & 69.01 & 10.18          & 13.10          & 3.23           & 67.20          & 28.78 & 30.99          & 54.73          & 8.46           & \textbf{55.90} & 14.81          & 43.28          & 77.88          & 5.72           \\ \midrule
Model Scale               & Dataset     & \multicolumn{5}{c|}{Amazon}                                               & \multicolumn{5}{c|}{SST-5}                                                & \multicolumn{5}{c}{SemEval}                                                        \\ \midrule
\multirow{6}{*}{T5-small} & Method      & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf           & ECE            & CErr$_{pos}$   & CErr$_{neg}$   \\ \cmidrule(l){2-17} 
                          & E-MLP       & 85.51          & 85.87 & \textbf{10.87} & \textbf{13.00} & 79.17          & 60.82          & 77.84 & \textbf{19.95} & \textbf{21.30} & 76.51          & 47.13          & 76.62          & \textbf{30.41} & \textbf{21.86} & 75.27          \\
                          & E-T5        & 85.51          & 63.09 & 15.18          & 19.73          & \textbf{4.31}  & 60.82          & 20.19 & 37.67          & 68.27          & 6.40           & 47.13          & 24.11          & 49.85          & 72.19          & 16.02          \\
                          & I-Vanilla   & 74.41          & 58.28 & 25.89          & 31.18          & 4.64           & 57.08          & 19.47 & 41.64          & 71.05          & 6.41           & 47.85          & 24.84          & 49.14          & 71.30          & 16.68          \\
                          & I-Iterative & \textbf{86.64} & 64.97 & 14.55          & 19.06          & 5.64           & \textbf{60.92} & 17.68 & 37.90          & 71.69          & 5.35           & \textbf{49.43} & 21.98          & 46.06          & 74.32          & 15.22          \\
                          & I-Multitask & 84.87          & 59.20 & 16.78          & 22.53          & 4.70           & 57.92          & 11.50 & 41.83          & 81.10          & \textbf{3.42}  & 48.65          & \textbf{15.41} & 49.94          & 80.43          & \textbf{8.41}  \\ \midrule
\multirow{6}{*}{T5-base}  & Method      & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf           & ECE            & CErr$_{pos}$   & CErr$_{neg}$   \\ \cmidrule(l){2-17} 
                          & E-MLP       & 89.19          & 89.82 & \textbf{6.92}  & \textbf{8.83}  & 78.70          & 67.67          & 81.30 & \textbf{15.72} & \textbf{17.30} & 78.37          & 55.02          & 79.01          & \textbf{24.05} & \textbf{19.45} & 77.13          \\
                          & E-T5        & 89.19          & 68.57 & 10.94          & 13.77          & 2.56           & 67.67          & 28.37 & 30.89          & 54.59          & 9.20           & 55.02          & 15.76          & 43.77          & 77.17          & 6.56           \\
                          & I-Vanilla   & 87.31          & 67.79 & 12.94          & 15.87          & \textbf{2.50}  & \textbf{65.51} & 24.90 & 33.68          & 59.76          & 6.96           & 51.50          & 15.26          & 47.71          & 78.96          & 6.62           \\
                          & I-Iterative & \textbf{90.65} & 69.70 & 9.82           & 12.20          & 3.28           & 67.10          & 20.65 & 32.25          & 64.03          & \textbf{5.01}  & \textbf{55.33} & \textbf{9.79}  & 44.08          & 85.07          & \textbf{4.25}  \\
                          & I-Multitask & 90.21          & 69.35 & 9.84           & 12.48          & 2.81           & 67.48          & 28.73 & 31.28          & 54.11          & 7.49           & \textbf{54.93} & 17.34          & 44.74          & 75.11          & 6.89           \\ \midrule
\multirow{6}{*}{T5-large} & Method      & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf  & ECE            & CErr$_{pos}$   & CErr$_{neg}$   & Acc            & Conf           & ECE            & CErr$_{pos}$   & CErr$_{neg}$   \\ \cmidrule(l){2-17} 
                          & E-MLP       & 91.14          & 91.65 & \textbf{4.89}  & \textbf{7.04}  & 78.18          & 69.17          & 83.16 & \textbf{17.31} & \textbf{15.40} & 79.94          & 54.35          & 77.30          & \textbf{22.95} & \textbf{21.60} & 75.99          \\
                          & E-T5        & 91.14          & 70.61 & 8.84           & 11.16          & 2.20           & 69.17          & 25.63 & 29.27          & 56.81          & 6.87           & 54.35          & 22.29          & 43.22          & 70.85          & 10.87          \\
                          & I-Vanilla   & 89.51          & 70.08 & 10.56          & 13.02          & \textbf{2.05}  & 68.98          & 24.66 & 29.46          & 57.82          & \textbf{6.30}  & 51.72          & 21.36          & 45.84          & 72.78          & \textbf{10.65} \\
                          & I-Iterative & \textbf{92.72} & 73.49 & 7.28           & 9.11           & 2.89           & \textbf{70.67} & 25.57 & 27.48          & 56.57          & 7.67           & \textbf{59.00} & 26.49          & 37.00          & 65.23          & 14.23          \\
                          & I-Multitask & 91.83          & 70.99 & 8.58           & 10.61          & 3.01           & 70.10          & 26.95 & 28.78          & 55.11          & 8.16           & 57.13          & 21.52          & 40.13          & 70.71          & 10.81          \\ \bottomrule
\end{tabular}

}


\label{tab:emergent_dev_size}
\end{table*}
